Solving the problem of overdetermination of quasisymmetric equilbrium solutions by near-axis expansions: I. Generalised force balance

It is well known that the process of construction of quasisymmetric magnetic fields in magnetostatic equilibrium with isotropic pressure suffers from the problem of overdetermination. This has led to the widespread belief that global quasisymmetric solutions are likely not to exist. We develop a general near-axis expansion procedure that does not rely on the assumption of magnetostatic equilibria with isotropic pressure. We then demonstrate that in equilibria with anisotropic pressure, it is possible to circumvent the problem of overdetermination and carry out the power-series solutions to higher order. This suggests, contrary to current belief, that the existence of globally quasisymmetric fields is likely if one relaxes the assumption of magnetostatic equilibria with isotropic pressure.

==> Figures/NAEGen.tex <==
\chapter{General near axis expansion for QS field}
\label{sec:NAEGen}
Let us briefly summarise the contents of the previous two paragraphs to motivate the main concern of the present chapter. In the first chapter, a construction of quasisymmetry from first principles was presented. As emphasised, this formulation is devoid of any consideration about the particular force balance the field is in. This concept of QS was initially proposed by \cite{burby2019}, with all previous considerations having focused on the special magnetostatic equilibrium case. \par
On a second chapter we applied this more general formulation to the magnetostatic case to see how the standard results come about with this new perspective. In particular, we rexplored briefly the near axis expansion \cite{garrenboozer1991a} construction, to see that in fact one is unable to carry it out to an order larger than second in the expansion parameter $\epsilon\propto\sqrt{\psi}$. The flux label is zero on axis, and one may consider the near axis expansion as a large aspect ratio one. \par
This failure comes to being as a result of an overdetermination of teh expansion. One finds that at subsequent orders, the number of equations that need to be satisfied exceeds that of new free functions. This observation has since \cite{garrenboozer1991b} been taken as not a definitive proof, but a strong indication that constructing a globally quasisymmetric system other than the truly symmetric cases might not be possible. \par
If one is to duck the lack of freedom in the near axis expansion, one should generally introduce some additional degree of freedom into the problem. We consider in this chapter the relaxation of the standard equilibrium magnetostatic balance $\n{j}\times\n{B}=\nabla p$ for a more general force. We shall especialise on the generalisation of the balance to that of anisotropic pressure, as is natural generalisation. Note that an arbitrary force on the RHS would affect the single particle Lagrangian, and thus probably the form of the force balance. \todo{What are the implications of these changes in the force balance on the Lagrangian? For instance, does anisotropy imply some E field that destroys QS?} \par
To possibly deal with this generalised situation, a mmore general construction of the near axis expansion is to be developed, and we do so in the first part of this chapter. As said, we shall then apply it to the case of anisotriopic equilibria, and to some particular cases such as that of a circular axis.

\section{General quasisymmetric near-axis expansion: magnetic equations} \label{NAEmagn}

\subsection{`Boozer-like' formulation of QS}
In order to implement effectively the quasisymmetric requirement into the expansion formulation, we shall try to cast it in as close as possible a form as the standard Boozer formulation. Just as a reminder, the standard approach states that for a field in magnetostatic equilibrium with well defined flux surfaces a field is QS iff one may write,
\begin{equation*}
    B=B(\psi,M\theta-N\phi),
\end{equation*}
where $\{\psi,\theta,\phi\}$ are taken to be Boozer coordinates, and $M,N\in\mathbb{Z}$.\todo{The coefficient $M=1$ taken for the better expansion. What if it is not?} The Boozer set assumes that $\n{j}\cdot\nabla\psi=0$, and provided this holds it has an associated Jacobian of the form,
\begin{equation}
    J=\frac{B_\phi+\iota B_\theta}{B^2} \label{eqn:jacCoord}
\end{equation}
where
\begin{equation*}
    \n{B}=B_\theta\nabla\theta+B_\phi\nabla\phi+B_\psi\nabla\psi,
\end{equation*}
and both $B_\phi$ and $N_\theta$ are flux functions. \par
Such a formulation of Qs is convenient to perform the expansion around the axis, as it allows for a reduced Taylor-Fourier series for $|\n{B}|$. Because a general force balance does not have an associated Boozer coordinate system, we encounter a problem. However, we shall show that one may construct a straight field line coordinate system that resembles it. \par
Let us start up by assuming the field to be constructed is quasisymmetric. And let us take as a starting point the formulation of QS introduced in Sec. \ref{boozerFormQS}: a field with well defined flux surfaces will be called quasisymmetric (in its \textit{weak} sense) iff there exists a straight field line coordinate system with a Jacobian $J=J(\psi,B)$ such that $B=B(\psi,M\theta+N\phi)$. \par
In this coordinate system, the Jacobian may be written in the same as (\ref{eqn:jacCoord}). However, generally one may not guarantee that the covariant functions will be flux functions. However, the particular condition on the Jacobian in our QS construction implies that the function
\begin{equation*}
    B_\alpha\equiv B_\phi+\iota B_\theta
\end{equation*}
is in fact $B_\alpha=B_\alpha(\psi,B)$. The construction of a Jacobian of the form given does in fact not exhaust all the straight field line angle choice freedom there is in the system. I.e., we may still transform coordinates using the gauge function $\omega$ to simplify things further, while preserving the nature of the Jacobian. \par
To mimic the Boozer form as close as possible, we would like to make $B_\alpha$ to be a flux function. This is in fact possible, and we show this explicitly in the following lines. Under the angular gauge transformation $\omega$, the old coordinates (primed quantities) map according to $\theta=\theta'+\iota\omega$ and $\phi=\phi'+\omega$. Under this mapping, the contravariant form of the magnetic field preserves its form, while the covariant form ttransforms,
\begin{align*}
    \n{B}=\left[B_{\theta'}\left(1-\iota\partial_\theta\omega\right)-B_{\phi'}\partial_\theta\omega\right]\nabla\theta+\left[-\iota B_{\theta'}\partial_\phi\omega+B_{\phi'}\left(1-\partial_\phi\omega\right)\right]\nabla\phi+\\
    +\left[B_{\psi'}-B_{\theta'}\partial_{\psi'}(\iota\omega)-B_{\phi'}\partial_\psi\omega\right]\nabla\psi.
\end{align*}
Thus, we may write,
\begin{equation*}
    \n{B}\cdot\nabla\omega=\frac{B^2}{B_\alpha}-\frac{B^2}{B_{\alpha'}},
\end{equation*}
which one could see just from how the Jacobian is to transform. Now, we want $B_\alpha=B_\alpha(\psi)$, and to see whether this is possible or not, we shall check two things. First that one may possibly solve for $\omega$ in the magnetic equation; and secondly that the Jacobian does not become singular or badly behaved. For the former, the solubility condition,
\begin{equation*}
    \langle\n{B}\cdot\nabla\omega\rangle=0=\left\langle\frac{B^2}{B_\alpha}\right\rangle-\left\langle\frac{B^2}{B_{\alpha'}}\right\rangle
\end{equation*}
\begin{equation*}
    B_\alpha=\frac{\langle B^2\rangle}{\langle B^2/B_{\alpha'}\rangle}.
\end{equation*}
So in fact one may transform coordinates in a way so as to make the $B_\alpha$ a flux function. It remains to be shown that the transformation does not vanish nor ddiverge. As a starting point, and by construction $J'\neq0$ was finite and smooth. As $B^2>0$ for a non-vanishing magnetic field (and thus so is its flux surface average), $B_\alpha$ \textbf{must} have the same sign as $J'$, and thus be non-zero. The same follows for the diverging behaviour. \par
Let us then summarise our QS formulation in this form: \textbf{a field with well defined flux surfaces is quasisymmetric iff there is a straight field line coordinate system in which the Jacobian has the form $J=B_\alpha(\psi)/B^2$ and the magnetic field magnitude $B=B(\psi,M\theta-N\phi)$.} Given this formulation, the covariant form of the magnetic field will be conveniently written as,
\begin{gather*}
    \n{B}=B_\theta\nabla\theta+(B_\alpha-\iota B_\theta)\nabla\phi+B_\psi\nabla\psi,
\end{gather*}
deprecating $B_\phi$ for $B_\alpha$. 

\subsection{Specifying the expansions}
Now that we have formulated QS in an efficient way, we write down the near axis exapnsions for the relevant functions in the system. \par
Before doing so, we shall introduce a last change of variables. In fact, we want to introduce the symmetry angle $\chi=\theta-N\phi$, where $N\in\mathbb{Z}$.\todo[]{M=1?} With this easy change of variables, the magnetic field can be written  
\begin{gather}
    \n{B}=B_\theta\nabla\chi+(B_\alpha-\Bar{\iota}B_\theta)\nabla\phi+B_\psi\nabla\psi= \nonumber\\
    =\nabla\psi\times\nabla\chi+\Bar{\iota}\nabla\phi\times\nabla\psi \label{eq:Bcocon}
\end{gather}
where $\Bar{\iota}=\iota-N$. With this set, conveniently, the magnetic field is constant along constant $\chi$ contours. We should check, just in case, what happens to the Jacobian of the coordinate system as a result of this latter change. Taking,
\begin{equation*}
    \nabla\psi\times\nabla\chi\cdot\nabla\phi=\nabla\psi\times\nabla(\theta-N\phi)\cdot\nabla\phi=\nabla\psi\times\nabla\theta\cdot\nabla\phi.
\end{equation*}
\par
Let us now expand our functions in this coordinate system, adopting the inverse problem. I.e., we are not to take $\{\psi,\chi,\phi\}$ as functions of spatial coordinates, but rather as parameters for the spatial coordinates themselves. With $\chi$ representing a poloidal angle, $\phi$ a toroidal one and $\psi$ a sort of radial coordinate we shall now proceed to expand functions. \par
Close to the axis, one may show that the flux coordinate $\psi\propto r^2$, and thus $\sqrt{\psi}$ is a sort of radial variable. In fact, to form an appropriate small parameter for the expansion, we will define $\epsilon=\sqrt{(\kappa_\mathrm{max})^2\psi/B_\mathrm{min}}$  as Garren and Boozer do in their procedure, where $B_\mathrm{min}$ is the minimum B field on axis, and $\kappa_\mathrm{max}$ the amximum curvature. This should guarantee the expansion coefficient to be dimensionless, and be truly small at all points around the axis when claimed small. Just for completeness, we would like to dnon-dimensionalise all the relevant expressions that have $\psi$ in it. This would imply $B_\alpha\rightarrow B_\alpha(\kappa_\mathrm{max})^2/B_\mathrm{min}$ and $B_\theta\rightarrow B_\theta()\kappa_\mathrm{max})^2/B_\mathrm{min}$. We shall from here on forget about these niceties and ignore these rescaled factors (i.e. $\psi=\epsilon^2$ for convenience). \par
 With this in mind, and in order to comply with regularity on axis (see \cite{landreman2018a}), a well behaved function can be expressed as a Taylor-Fourier series,
\begin{equation}
    f(\psi,\theta,\phi)=\sum_n\epsilon^n{\sum_m^{n}}\left[f_{nm}^c(\phi)\cos m\chi+f_{nm}^s(\phi)\sin m\chi\right], \label{eq:generalExpansion}
\end{equation}
where the second sum is over even or odd indices, depending on $n$. The regularity requirement is clear in that a given $\chi$ harmonic $m$ will appear to lowest order with a power of $\epsilon^m$.  \par
The class of functions that are to be considered flux functions will be expanded as,
\begin{equation}
    f(\psi)=\sum_{n=0}^\infty\epsilon^{2n}f_n
\end{equation}
where $f_n$ coefficients are constant. From our magnetic field formulation, $\Bar{\iota}$ and $B_\alpha$ by construction are flux functions. \par
A second class of functions are those that have the symmetry of the magnetic field. In fact, we shall for convenience deal with the expansion of
\begin{equation}
    \frac{1}{B^2}=B_0+\sum_{n=1}^\infty\epsilon^n \sum_{m=0|1}^n\left(B_{nm}^c\cos m\chi +B_{nm}^s\sin m\chi\right),
\end{equation}
where, again, the $B_{nm}^{c/s}$ are constants. \par
Finally, we have the set of functions with no particular constraint on their dependence, but just that they are well-behaved functions of space. This is the case with the inverse map functions. Here we adopt the Frenet basis (some more details in the next subsection) to express this inverse mapping in the vein of \cite{garrenboozer1991a}, even  with the limitations of such a set. A procedure with cylindrical coordinates as in \cite{landreman2018a} is left for later. Now, writing $\n{x}=\n{r}_0+X\hat{\n{\kappa}}_0+Y\hat{\n{\tau}}_0+Z\hat{\n{b}}_0$, the functions $X$, $Y$ and $Z$ will be expanded as in (\ref{eq:generalExpansion}). The same is true for the functions $B_\theta$ and $B_\psi$. \par
As a reminder of the difference with the standard approach like in \cite{garrenboozer1991b}, here $B_\theta$ is not a flux function, but rather a fully spatially dependent function. As for $B_\psi$, in magnetostatics $B_\psi$ has the same angular dependence as $B^2$, and therefore in a QS field, it would have an expansion similar to that of $1/B^2$. However, this behavious is inhereted from the force balance, and therefore at this level must be dropped in favour of the most general behaviour. \par
These functions and expansions complete the set of functions to describe the magnetic field, and will requitre of no additional function until a particular form of force balance is considered. 

\subsection{Expansion procedure: magnetic field equations}
The quasisymmetric magnetic field must satisfy two  main equations close to the axis, and these will be our concern here. However, before getting there, we must complete the picture of the inverse mapping by obtaining a number of necessary expressions. Defining $\n{x}=\n{r}_0+X\hat{\n{\kappa}}_0+Y\hat{\n{\tau}}_0+Z\hat{\n{b}}_0$, we need to obtain closed forms for the partial derivatives with respect to our straight field line coordinate system. At this point, this is not different from \cite{garrenboozer1991a}, and some algebra, and the definitions of curvature and torsion,
\begin{gather*}
    \frac{\mathrm{d}\n{r}_0}{\mathrm{d}l}=\n{b}_0 \\
    \frac{\mathrm{d}\hat{\n{b}}_0}{\mathrm{d}l}=\kappa(l)\hat{\kappa}_0 \\
    \frac{\mathrm{d}\hat{\kappa_0}}{\mathrm{d}l}=-\kappa(l)\hat{\n{b}}_0-\tau(l)\hat{\tau}_0 \\
    \frac{\mathrm{d}\hat{\tau}_0}{\mathrm{d}l}=\tau(l)\hat{\kappa}_0
\end{gather*}
where $l$ parametrises the length along the magnetic axis, to give
\begin{subequations}
    \begin{gather}
        \frac{\partial \n{x}}{\partial\psi} = \partial_\psi X\hat{\kappa}_0+\partial_\psi Y\hat{\tau}_0+\partial_\psi Z\hat{\n{b}}_0 \\
        \frac{\partial\n{x}}{\partial \chi} = \partial_\chi X\hat{\kappa}_0+\partial_\chi Y\hat{\tau}_0+\partial_\chi Z\hat{\n{b}}_0 \\
        \frac{\partial\n{x}}{\partial \phi} = \left(\partial_\phi X+\tau Y\frac{\mathrm{d}l}{\mathrm{d}\phi}+Z\kappa\frac{\mathrm{d}l}{\mathrm{d}\phi}\right)\hat{\kappa}_0+\left(\partial_\phi Y-X\tau\frac{\mathrm{d}l}{\mathrm{d}\phi}\right)\hat{\tau}_0+\left(\partial_\phi Z-X\kappa\frac{\mathrm{d}l}{\mathrm{d}\phi}+\frac{\mathrm{d}l}{\mathrm{d}\phi}\right)\hat{\n{b}}_0.
    \end{gather}
\end{subequations}
With this, let us write down our $\n{B}$ field relevant equations.

\subsubsection{Jacobian equation}
Let us start by focusing on the Jacobian equation. This is in fact a way in which the spatial functions are related to the magnetic field magnitude, on top of which the QS conditions are imposed via the reduced form of its Taylor-Fourier expansion, as presented above. \par
There is no unique way of doing this. However, let us use the fact that $J=B_\alpha^2/B^2$ in our Boozer-like coordinate system. On top, we shall try to minimise the amount of algebraic clutter. Similarly to \cite{garrenboozer1991a}, and using the dual relations of the form $\nabla\psi\times\nabla\chi=J^{-1}\partial\n{x}/\partial\phi$, we may write
\begin{equation}
    \frac{B_\alpha^2}{B^2}=\left|\frac{\partial\n{x}}{\partial \phi}+\Bar{\iota}\frac{\partial\n{x}}{\partial \chi}\right|^2.
\end{equation} 
Explicitly, using the Taylor-Fourier expansions relevant, we may write
\begin{align}
    \frac{B_\alpha^2}{B^2}=\left(\Bar{\iota}\partial_\chi X+\partial_\phi X+\tau Y\frac{\mathrm{d}l}{\mathrm{d}\phi}+Z\kappa\frac{\mathrm{d}l}{\mathrm{d}\phi}\right)^2+\left(\Bar{\iota}\partial_\chi Y+\partial_\phi Y-X\tau\frac{\mathrm{d}l}{\mathrm{d}\phi}\right)^2+\nonumber\\
    +\left(\Bar{\iota}\partial_\chi Z+\partial_\phi Z-X\kappa\frac{\mathrm{d}l}{\mathrm{d}\phi}+\frac{\mathrm{d}l}{\mathrm{d}\phi}\right)^2 \label{eq:Jgen}
\end{align}
With this equation at hand we are ready to introduce explicitly the expansion form for the various functions, and analyse the resultant equations order by order. This is usually done in two steps. First, considering the Taylor expansion in $\epsilon$, before explicitly introducing the Fourier series. This allows in many places to identify ways to simplify the equations that in the fully explicit form would be difficult to do. After doing so, we may substitute the whole Fourier explicit expression. 

\paragraph{Order $\epsilon^0$}:
\begin{equation}
    J^0:~~~~~~B_{\alpha 0}=\frac{\mathrm{d}l}{\mathrm{d}\phi}\frac{1}{\sqrt{B_0}}
\end{equation}
This implies that, as both $B_{\alpha0}$ and $B_0$ are constants by construction, so must $\mathrm{d}l/\mathrm{d}\phi$. Said differently, $l\propto\phi$. This is in fact consistent with the MS approach in \cite{garrenboozer1991b}.

\paragraph{Order $\epsilon^1$}: 
\begin{equation*}
    J^1:~~~~~~-2\left(\frac{\mathrm{d}l}{\mathrm{d}\phi}\right)^2X_1\kappa=B_{\alpha0}^2B_1
\end{equation*}
This may be rewritten explicitly as an expression defining $X_1$,
\begin{equation*}
    X_1=-\frac{B_1}{2B_0}\frac{1}{\kappa}.
\end{equation*}
The harmonic components can then just be read off,
\begin{gather}
    X_{11}^C=\frac{\eta}{\kappa} \\
    X_{11}^S=0
\end{gather}
where $\eta=-B_{11}^C/2B_0$. We have chosen by construction $B_{11}^S=0$, which is in fact equivalent to choosing the offset of our angular coordinates, given that the magnetic coefficients are constant (so in fact equivalent to a constant phase offset). This is just a convenient choice. \par
Importantly, all the angular dependence of $X_{11}^C\propto1/\kappa(\phi)$ occurs through the curvature of the magnetic axis. In particular, as $\kappa\rightarrow0$, the function has a $1/\kappa$ divergence. Physically this means that in the limit of a locally straight axis, the flux surfaces get stretched along the direction of teh curvature, and in the limit, it becomes a flat ribbon. As pointed in \cite{garrenboozer1991b}, this requires the magnetic axis to have a non-vanishing curvature all along the axis. It is a simple picture to bear in mind: if one straightens the axis, to keep the quasisymmetry of the field, the flux surfaces would be stretched in the curvature direction, and shrink in the binormal direction. When we look at $Y$ and how it behaves, we will see that it is in fact consistent with this sketched squashing. 

\paragraph{Order $\epsilon^2$}: 
\begin{align*}
   J^2:~~~~~ 2\left(\frac{\mathrm{d}l}{\mathrm{d}\phi}\right)^2\kappa X_2=-2B_{\alpha0}B_{\alpha1}B_0-B_{\alpha0}^2B_{2}+\left(\frac{\mathrm{d}l}{\mathrm{d}\phi}\right)^2X_1^2\kappa^2+2\left(\frac{\mathrm{d}l}{\mathrm{d}\phi}\right)Z_2'
    +\\
    +\left(\frac{\mathrm{d}l}{\mathrm{d}\phi}Y_1\tau+X_1'+\Bar{\iota}_0\Dot{X}_1\right)^2+\left(-\frac{\mathrm{d}l}{\mathrm{d}\phi}X_1\tau+Y_1'
    +\Bar{\iota}_0\Dot{Y}_1\right)^2+2\left(\frac{\mathrm{d}l}{\mathrm{d}\phi}\right)\Bar{\iota}_0\Dot{Z}_2
\end{align*}
where the prime denotes a derivative with respect to $\phi$ and a dot a derivative with respect to $\chi$. Just for completeness, the explicit form for the components of $X_2$ are as follow. 
\begin{align*}
X^C_{2,0}{}&= \frac{1}{4 l^2 \kappa {}}\left[-2 B_{\alpha0}^2 B^C_{2,0}+l^2 \kappa {}^2 X^C_{1,1}{}{}^2+l^2 \tau {}^2 X^C_{1,1}{}{}^2+l^2 \tau {}^2 Y^C_{1,1}{}{}^2+\right.\\
&\left.+l^2 \tau {}^2 Y^S_{1,1}{}{}^2+2 l \tau {} Y^C_{1,1}{} X^C_{1,1}{}'-2 l \tau {} X^C_{1,1}{} Y^C_{1,1}{}'-2 \Bar{\iota} _0 \left(2 l \tau {} X^C_{1,1}{} Y^S_{1,1}{}-Y^S_{1,1}{} Y^C_{1,1}{}'+\right.\right.\\
&\left.\left.+Y^C_{1,1}{} Y^S_{1,1}{}'\right)+4 l Z^C_{2,0}{}'+\Bar{\iota} _0^2 \left(X^C_{1,1}{}{}^2+Y^C_{1,1}{}{}^2+Y^S_{1,1}{}{}^2\right)+X^C_{1,1}{}'{}^2+\right.\\
&\left.+Y^C_{1,1}{}'{}^2+Y^S_{1,1}{}'{}^2-4 B_0 B_{\alpha1} B_{\alpha0}\right]
\end{align*}
\begin{align*}
 X^C_{2,2}{}&= \frac{1}{4 l^2 \kappa {}}\left[-2 B^C_{2,2} B_{\alpha0}^2+l^2 \kappa {}^2 X^C_{1,1}{}{}^2+l^2 \tau {}^2 X^C_{1,1}{}{}^2+l^2 \tau {}^2 Y^C_{1,1}{}{}^2-\right.\\
 &\left.-l^2 \tau {}^2 Y^S_{1,1}{}{}^2+X^C_{1,1}{}'{}^2+Y^C_{1,1}{}'{}^2-Y^S_{1,1}{}'{}^2-\Bar{\iota} _0^2 \left(X^C_{1,1}{}{}^2+Y^C_{1,1}{}{}^2-Y^S_{1,1}{}{}^2\right)+\right.\\
 &\left.+2 l \tau {} Y^C_{1,1}{} X^C_{1,1}{}'-2 l \tau {} X^C_{1,1}{} Y^C_{1,1}{}'+2 \Bar{\iota} _0 \left(4 l Z^S_{2,2}{}+Y^S_{1,1}{} Y^C_{1,1}{}'+Y^C_{1,1}{} Y^S_{1,1}{}'\right)+4 l Z^C_{2,2}{}'\right]
\end{align*}
\begin{align*}
X^S_{2,2}{}&= \frac{1}{2 l^2 \kappa {}}\left[-B_{\alpha0}^2 B^S_{2,2}+l^2 \tau {}^2 Y^C_{1,1}{} Y^S_{1,1}{}-\Bar{\iota} _0 \left(4 l Z^C_{2,2}{}+X^C_{1,1}{} X^C_{1,1}{}'+Y^C_{1,1}{} Y^C_{1,1}{}'-\right.\right.\\
&\left.\left.-Y^S_{1,1}{} Y^S_{1,1}{}'\right)+l \tau {} Y^S_{1,1}{} X^C_{1,1}{}'-l \tau {} X^C_{1,1}{} Y^S_{1,1}{}'+\right.\\
&\left.+2 l Z^S_{2,2}{}'-\iota _0^2 Y^C_{1,1}{} Y^S_{1,1}{}+Y^C_{1,1}{}' Y^S_{1,1}{}'\right]
\end{align*}
We have here used the shorthand $l$ for $\mathrm{d}l/\mathrm{d}\phi$ which should not be confused, and has just been adopted for the economy of notation. One could rewrite these expressions by factoring out terms of the RHS, but we shall not be concerned with this here, and just leace the equations as they are, which we simply wrote for completeness.

\paragraph{Higher orders}: having explicitly looked at the first couple of orders, we may extrapolate how these equations may be used to arbitrary order $n$. Equation $J^n$ will give a closed form for $X_n$ in terms of other functions. This is true to any order thanks to the third parenthesis term in (\ref{eq:Jgen}). The square yields a term with an isolated $X$ multiplied by no other function $X,Y$ or $Z$. This is what makes solving for $X_n$ always possible and simple. In fact, an account of the functions and orders shows that
\begin{equation}
    J^n(\epsilon^n):~~~~~~X_n\mapsto Z_n, Y_{n-1}, B_n.
\end{equation}
So, at each order one obtains $n+1$ independent equations from each of the harmonmic components, and thus we may understand the set of $J$ equations to describe the function $X$. \par
To summarise these dependencies from the Jacobian equation, and refer in a succint way to what is to be solved at each order based on what knowledge, we introduce the diagram in Fig. \ref{fig:JeqDiag}. The arrows represent the dependency, while the shaded function in green indicates the function to be solved for.
\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figures/Chapter3/JeqDiag.jpg}
    \caption{\textbf{Diagram for the Jacobian equation $J^n$.} The green shaded circle represents the function that one should solve the equation for ($X_n$). The arrows indicate the leading order of the functions needed to find such a solution.}
    \label{fig:JeqDiag}
\end{figure}

\subsubsection{Co(ntra)variant equation}
The co(ntra)variant vector equation relates the covariant and contravariant forms of the magnetic field as written in (\ref{eq:Bcocon}). It is straightforward to write, using the dual relations of a form like $\nabla\psi\times\nabla\chi=J^{-1}\partial\n{x}/\partial\phi$ and $\nabla\phi=J^{-1}\partial\n{x}/\partial\psi\times\partial\n{x}/\partial\chi$,
\begin{equation}
    (B_\alpha-\Bar{\iota}B_\theta)\frac{\partial\n{x}}{\partial\psi}\times\frac{\partial\n{x}}{\partial\chi}+B_\theta\frac{\partial\n{x}}{\partial\phi}\times\frac{\partial\n{x}}{\partial\psi}+B_\psi\frac{\partial\n{x}}{\partial\chi}\times\frac{\partial\n{x}}{\partial\phi}=\frac{\partial\n{x}}{\partial\phi}+\Bar{\iota}(\psi)\frac{\partial\n{x}}{\partial\chi}. \label{eq:co(ntra)variant}
\end{equation}
This equation mainly includes information about the existence of flux surfaces and the divergenceless nature of the magnetic field. \par
Given this equation, take the machinery and turn the handle to write the three Frenet components of the equation. The $\hat{\n{b}}_0$ component,
\begin{align}
    &-(B_\alpha-\bar{\iota}B_\theta)\left(\partial_\chi X\partial_\psi Y-\partial_\psi X\partial_\chi Y\right)-\nonumber\\
    &-B_\psi\left[\partial_\chi Y\left(\partial_\phi X+\tau Y\frac{\mathrm{d}l}{\mathrm{d}\phi}+Z\kappa\frac{\mathrm{d}l}{\mathrm{d}\phi}\right)-\partial_\chi X\left(\partial_\phi Y-X\tau\frac{\mathrm{d}l}{\mathrm{d}\phi}\right)\right]+\nonumber\\
    &+B_\theta\left[\partial_\psi Y\left(\partial_\phi X+\tau Y\frac{\mathrm{d}l}{\mathrm{d}\phi}+Z\kappa\frac{\mathrm{d}l}{\mathrm{d}\phi}\right)-\partial_\psi X\left(\partial_\phi Y-X\tau\frac{\mathrm{d}l}{\mathrm{d}\phi}\right)\right]=\nonumber\\
    &=\left(\partial_\phi Z-X\kappa\frac{\mathrm{d}l}{\mathrm{d}\phi}+\frac{\mathrm{d}l}{\mathrm{d}\phi}\right)+\Bar{\iota}\partial_\chi Z, \label{eq:Cb}
\end{align}
the $\hat{\kappa}_0$ component,
\begin{align}
    &-(B_\alpha-\bar{\iota}B_\theta)\left(\partial_\chi Y\partial_\psi Z-\partial_\psi Y\partial_\chi Z\right)-\nonumber\\
    &-B_\psi\left[\partial_\chi Z\left(\partial_\phi Y-X\tau\frac{\mathrm{d}l}{\mathrm{d}\phi}\right)-\partial_\chi Y\left(\partial_\phi Z-X\kappa\frac{\mathrm{d}l}{\mathrm{d}\phi}+\frac{\mathrm{d}l}{\mathrm{d}\phi}\right)\right]+\nonumber\\
    &+B_\theta\left[\partial_\psi Z\left(\partial_\phi Y-X\tau\frac{\mathrm{d}l}{\mathrm{d}\phi}\right)-\partial_\psi Y\left(\partial_\phi Z-X\kappa\frac{\mathrm{d}l}{\mathrm{d}\phi}+\frac{\mathrm{d}l}{\mathrm{d}\phi}\right)\right]=\nonumber\\
    &=\left(\partial_\phi X+\tau Y\frac{\mathrm{d}l}{\mathrm{d}\phi}+Z\kappa\frac{\mathrm{d}l}{\mathrm{d}\phi}\right)+\Bar{\iota}\partial_\chi X, \label{eq:Ck}
\end{align}
and the $\hat{\tau}_0$ component,
\begin{align}
    &-(B_\alpha-\bar{\iota}B_\theta)\left(\partial_\chi Z\partial_\psi X-\partial_\psi Z\partial_\chi X\right)-\nonumber\\
    &-B_\psi\left[\partial_\chi X\left(\partial_\phi Z-X\kappa\frac{\mathrm{d}l}{\mathrm{d}\phi}+\frac{\mathrm{d}l}{\mathrm{d}\phi}\right)-\partial_\chi Z\left(\partial_\phi X+\tau Y\frac{\mathrm{d}l}{\mathrm{d}\phi}+Z\kappa\frac{\mathrm{d}l}{\mathrm{d}\phi}\right)\right]+\nonumber\\
    &+B_\theta\left[\partial_\psi X\left(\partial_\phi Z-X\kappa\frac{\mathrm{d}l}{\mathrm{d}\phi}+\frac{\mathrm{d}l}{\mathrm{d}\phi}\right)-\partial_\psi Z\left(\partial_\phi X+\tau Y\frac{\mathrm{d}l}{\mathrm{d}\phi}+Z\kappa\frac{\mathrm{d}l}{\mathrm{d}\phi}\right)\right]=\nonumber\\
    &=\left(\partial_\phi Y-X\tau\frac{\mathrm{d}l}{\mathrm{d}\phi}\right)+\Bar{\iota}\partial_\chi Y. \label{eq:Ct}
\end{align}
It is imprtant to note the structure in these equations, as the expressions in rounded parenthesis reapeat in the different components. One would thus expect that particular combinations of these equations would lead to simplified expressions. These equations will be referred to in shorthand as $C_b$ or $C_\perp$ (thet latter involves both \ref{eq:Ck} and \ref{eq:Ct}, as they usually come in together). \par
This is not the only way in which one could write this set of equations. As a matter of fact, one could project the original vector equation in alternative directions other than the Frenet basis set. For completeness, we include two alternative forms that will result useful at soome point in the expansion construction. These forms express the covariant functions $B_\psi$ and $B_\theta$ in terms of the spatial functions in the following way,
\begin{align}
    B_\psi J=&\partial_\psi X\left(\partial_\phi X+\tau Y\frac{\mathrm{d}l}{\mathrm{d}\phi}+Z\kappa\frac{\mathrm{d}l}{\mathrm{d}\phi}+\Bar{\iota}\partial_\chi X\right)+\partial_\psi Y\left(\partial_\phi Y-X\tau\frac{\mathrm{d}l}{\mathrm{d}\phi}+\Bar{\iota}\partial_\chi Y\right)+\nonumber\\
    &+\partial_\psi Z\left(\partial_\phi Z-X\kappa\frac{\mathrm{d}l}{\mathrm{d}\phi}+\frac{\mathrm{d}l}{\mathrm{d}\phi}+\Bar{\iota}\partial_\chi Z\right) \label{eq:alterC1}
\end{align}
and
\begin{align}
    B_\theta J=&\partial_\chi X\left(\partial_\phi X+\tau Y\frac{\mathrm{d}l}{\mathrm{d}\phi}+Z\kappa\frac{\mathrm{d}l}{\mathrm{d}\phi}+\Bar{\iota}\partial_\chi X\right)+\partial_\chi Y\left(\partial_\phi Y-X\tau\frac{\mathrm{d}l}{\mathrm{d}\phi}+\Bar{\iota}\partial_\chi Y\right)+\nonumber\\
   & +\partial_\chi Z\left(\partial_\phi Z-X\kappa\frac{\mathrm{d}l}{\mathrm{d}\phi}+\frac{\mathrm{d}l}{\mathrm{d}\phi}+\Bar{\iota}\partial_\chi Z\right). \label{eq:alterC2}
\end{align}
These equations can be obtained by dotting the (\ref{eq:co(ntra)variant}) equation with $\partial\n{x}/\partial\psi$ and $\partial\n{x}/\partial\chi$ respectively. The forms for $B_\theta$ and $B_\psi$ are very close to one another, something that will prove important in what is to come. \par
With the equations (\ref{eq:Cb})-(\ref{eq:Ct}) at hand, we should now look order by order at the equations thereby obtained. We shall look at the lower order equations explicitly, finally to suggest how it would generalise to arbitrary order $n$. Note that the equations will closely resemble those in the usual \cite{garrenboozer1991b} construction, with the only difference that $B_\theta$ is not necessarily a flux function in our case.

\paragraph{Order $\epsilon^{-1}$}: the $C_\perp$ equations have a leading $\epsilon^{-1}$ order, due to the flux derivatives in these equations. One writes,
\begin{gather*}
    C_\kappa^{-1}:~~~~-B_{\theta0}\frac{\mathrm{d}l}{\mathrm{d}\phi}Y_1=0 \\
    C_\tau^{-1}:~~~~-B_{\theta0}\frac{\mathrm{d}l}{\mathrm{d}\phi}X_1=0.
\end{gather*}
Both these equations are satisfied if we were to take
\begin{equation}
    B_{\theta0}=0.
\end{equation}
We have assumed that neither $X_1$, $Y_1$ nor $\mathrm{d}l/\mathrm{d}\phi$ vanish trivially. In the magnetostatic case this would be equivalent to the claim that there is no delta shaped current flowing toroidally along the magnetic axis. \todo{What if we take the trivial solution for the position functions?}

\paragraph{Order $\epsilon^0$}:
\begin{gather*}
    C_b^0:~~~~-2\frac{\mathrm{d}l}{\mathrm{d}\phi}+B_{\alpha0}\left(X_1\partial_\chi Y_1-Y_1\partial_\chi X_1\right)=0 \\
    C_\kappa^0:~~~~-B_{\theta1}\frac{\mathrm{d}l}{\mathrm{d}\phi} Y_1+B_{\alpha0}\left(Y_1\partial_\chi Z_1-Z_1\partial_\chi Y_1\right)=0 \\
    C_\tau^0:~~~~B_{\theta1}\frac{\mathrm{d}l}{\mathrm{d}\phi} X_1+B_{\alpha0}\left(Z_1\partial_\chi X_1-X_1\partial_\chi Z_1\right)=0 
\end{gather*}
Combininng the latter two to eliminate $B_{\theta1}$, and applying $C_b^0$, one finds that,
\begin{equation}
    Z_1\frac{\mathrm{d}l}{\mathrm{d}\phi}=0\rightarrow Z_1=0
\end{equation}
and therefore,
\begin{equation}
    B_{\theta1}=0.
\end{equation}
The other only remaining equation is $C_b^0$. Using the expansions for the spatial functions, we may recast this condition in the form,
\todo{When introduced Y say something about the squashing, perhaps the elliptical nature}
\begin{equation}
    Y_{11}^S=\frac{2\sqrt{B_0}}{\eta}\kappa.
\end{equation}
Thus, as the curvature on axis becomes smaller and smaller, we expect the flux surfaces close to the magnetic axis to get squeezed in the direction of the binormal $\hat{\tau}$. As we saw before, the surface becomes elongated along the curvature region. Thus, in fact, the magnetic surfaces become squeezed (tending towards a ribbon) as the magnetic axis straightens, an unavoidable result for quasisymmetric fields (as they do not depend on the particular force balance in consideration).

\paragraph{Order $\epsilon^1$}: let us start by focusing on the $C_\perp^1$ equations, leaving the $b$ component for later. We may write,
\begin{align*}
    C_\kappa^1:~~~~~-B_{\theta2}\frac{\mathrm{d}l}{\mathrm{d}\phi}Y_1+2B_{\psi0}\frac{\mathrm{d}l}{\mathrm{d}\phi}\partial_\chi Y_1-B_{\alpha0}(2Z_2\partial_\chi Y_1-Y_1\partial_\chi Z_2)=\\
    =2\left(\frac{\mathrm{d}l}{\mathrm{d}\phi}\tau Y_1+\partial_\phi X_1+\Bar{\iota}_0\partial_\chi X_1\right)
\end{align*}
\begin{align*}
    C_\tau^1:~~~~~B_{\theta2}\frac{\mathrm{d}l}{\mathrm{d}\phi}X_1-2B_{\psi0}\frac{\mathrm{d}l}{\mathrm{d}\phi}\partial_\chi X_1+B_{\alpha0}(2Z_2\partial_\chi X_1-X_1\partial_\chi Z_2)=\\
    =2\left(-\frac{\mathrm{d}l}{\mathrm{d}\phi}\tau X_1+\partial_\phi Y_1+\Bar{\iota}_0\partial_\chi Y_1\right).
\end{align*}
The largest order functions in these equations are $Z_2$ and $B_{\theta2}$, and so it would seem that we should try to recast the equations so as to obtain expressions for these functions.\par
Multiplying $C_\kappa^1$ by $X_1$ and $C_\tau^1$ by $Y_1$, adding both equations together, and applying our knowledge from $C_b^0$,
\begin{equation}
    Z_2=\sqrt{B_0}B_{\psi0}-\left(\frac{\mathrm{d}l}{\mathrm{d}\phi}\right)^{-1}(\partial_\phi+\Bar{\iota}_0\partial_\chi)\left(\frac{X_1^2+Y_1^2}{4}\right).
\end{equation}
Note here that $Z_2$ depends on $B_{\psi0}$, a function of the toroidal angle $\phi$. Its particular form is determined by force balance, as it is evident in teh magnetostatic case in which $B_\psi$ has the same angular dependence as $1/B^2$. While $B_{\psi0}$ is here not subject to any constraint, we shall see when force balance is explored that its appearence is in fact quite very important.\par
From this form, we could straightforwardly obtain the form Fouriered form of the different harmonic components of $Z_2$. These are in fact identical to those obtained in \cite{garrenboozer1991a}, and thus we shall simply write them down for completeness,
\begin{gather*}
    Z_{2,0}=\frac{\mathrm{d}l}{\mathrm{d}\phi}\frac{B_{\psi0}}{B_{\alpha0}}-\frac{1}{8}\left(\frac{\mathrm{d}l}{\mathrm{d}\phi}\right)^{-1}\frac{\mathrm{d}V_1}{\mathrm{d}\phi} \\
    Z_{2,2}^C=-\frac{1}{8}\left(\frac{\mathrm{d}l}{\mathrm{d}\phi}\right)^{-1}\left[\frac{\mathrm{d}V_3}{\mathrm{d}\phi}+2\Bar{\iota}_0V_2\right] \\
    Z_{2,2}^S=-\frac{1}{8}\left(\frac{\mathrm{d}l}{\mathrm{d}\phi}\right)^{-1}\left[\frac{\mathrm{d}l}{\mathrm{d}\phi}-2\Bar{\iota}_0V_3\right]
\end{gather*}
where,
\begin{gather*}
    V_1 = (X_{1,1}^C)^2+(Y_{1,1}^C)^2+(Y_{1,1}^S)^2 \\
    V_2 = 2Y_{1,1}^CY_{1,1}^S \\
    V_3 = (X_{1,1}^C)^2+(Y_{1,1}^C)^2-(Y_{1,1}^S)^2.
\end{gather*}
This construction of $Z_2$ uses up three constraint equation. So we have three additional equations left. To see what the remaining equations are, we may substitute the freshly obtained forms for $Z_2$ into either equation $C_\kappa^1$ or $C_\tau^1$, and look at the obtained equations. From the previous argument, one could expect to treat these remaining equations as equations for $B_{\theta2}$. We shall see how this is true or not. \par
Two of the components, the largest harmonics,
\begin{gather*}
    0=B_{\theta22}^SX_{11}^C+B_{\theta22}^CX_{11}^S \\
    0=B_{\theta22}^CX_{11}^C-B_{\theta22}^SX_{11}^S,
\end{gather*}
from which it follows that
\begin{equation}
    B_{\theta22}=0.
\end{equation}
A last equation that one may in fact obtain here is,
\begin{align*}
    \frac{\mathrm{d}l}{\mathrm{d}\phi}(2\tau+B_{\theta20})X_{11}^C X_{11}^S+\Bar{\iota}_0 (X_{11}^C Y_{11}^C-X_{11}^S Y_{11}^S)-(X_{11}^S Y_{11}^{C\prime}+X_{11}^C Y_{11}^{S\prime})-\\
    -\frac{1}{2\sqrt{B_0}}\left\{\Bar{\iota}_0[(X_{11}^C)^2+(X_{11}^S)^2](X_{11}^C X_{11}^S+Y_{11}^C Y_{11}^S)+(X_{11}^S)^2(X_{11}^C X_{11}^{C\prime}+Y_{11}^C Y_{11}^{C\prime})-\right.\\
    \left.    -(X_{11}^C)^2 (X_{11}^S X_{11}^{S\prime}+Y_{11}^S Y_{11}^{S\prime})\right\}=0.
\end{align*}
As expected, the equation includes $B_{\theta20}$, which is generally some function of $\phi$. Thus this equation might be interpreted as an equation for $B_{\theta20}$ or instead a differential equation for $Y_{11}^C$. It is the case that the latter interpretation is more appropriate, and when specific forms of the force balance equation are considered will be more clear. It could help to understand this choice the fact that we shall be able to cast the force balance equations (in the cases of magnetostatic equilibrium and anisotropic pressure) in a form independent of the functions $X,~Y$ and $Z$. Therefore, taking this equation as an ODE is in fact necessary. One could rewrite the equation in the following form,
 \begin{align*}
    (Y_{11}^C)'-Y_{11}^C\frac{\kappa'}{\kappa}+&(Y_{11}^C)^2\frac{\Bar{\iota}_0\eta}{2\sqrt{B_0}\kappa}+\Bar{\iota}_0\left(\frac{2\sqrt{B_0}}{\eta}\kappa+\frac{\eta^3}{2\sqrt{B_0}}\frac{1}{\kappa^3}\right)-\\
    &-\frac{\mathrm{d}l}{\mathrm{d}\phi}(2\tau+B_{\theta20})\frac{\eta}{\kappa}=0.
 \end{align*}
 Defining $Y_{11}^C=Y_{11}^S\sigma$, this equation reduces to,
 \begin{equation}
     \frac{\mathrm{d}\sigma}{\mathrm{d}\phi}=-\Bar{\iota}_0\left[1+\frac{1}{4B_0}\left(\frac{\eta}{\kappa}\right)^4+\sigma^2\right]+\frac{B_{\alpha0}}{2}(2\tau+B_{\theta20})\left(\frac{\eta}{\kappa}\right)^2.
 \end{equation}
This is a first order non-linear differential equation to be solved for $\sigma$ subject to periodic boundary conditions $\sigma(0)=\sigma(2\pi)$, which should specify the problem uniquely. We insist here that $B_{\theta20}$ is some unknown function of $\phi$ at this point, and we will not be able to resolve this until some specific force balance is introduced. It will then be clear why this differential equation should be taken to be an equation for $\sigma$. An equation of this form has been obtained previously in \cite{garrenboozer1991b} or \cite{landreman2018a}, and the structure of the equation and existence of periodic solutions discussed. We refer to these for more details. We should point out as a point of difference, that in the present formulation $B_{\theta20}$ is not a constant but a function of $\phi$.  \par
Summarising what we obtained from $C_\perp^1$: we constructed explicitly $Z_2$ in terms of known functions, $Y_{11}^C$ and $B_{\psi0}$, obtained a differential equation for $Y_{11}^C$ and pinned down two of the components of $B_{\theta2}$. \par
Let us now turn our view onto $C_b^1$, and write
\begin{align*}
   C_b^1:~~~~ 2\frac{\mathrm{d}l}{\mathrm{d}\phi}X_1\kappa=B_{\alpha0}(2Y_2\partial_\chi X_1+Y_1\partial_\chi X_2-2X_2\partial_\chi Y_1-X_1\partial_\chi Y_2).
\end{align*}
Looking at the harmonic components of the equation, we are able to write
\begin{gather}
    Y_{22}^C=Y_{20}-\frac{1}{B_{\alpha0}}\frac{\beta}{X_{11}^C} \\
    Y_{22}^S=-\frac{1}{B_{\alpha0}}\frac{\alpha}{X_{11}^C}
\end{gather}
\begin{gather*}
    \alpha=\frac{\mathrm{d}l}{\mathrm{d}\phi}\kappa X_{11}^C-B_{\alpha0}( X_{22}^S Y_{11}^C- X_{20}^C Y_{11}^S- X_{22}^C Y_{11}^S) \\
    \beta=-B_{\alpha0}( X_{22}^C Y_{11}^C- X_{20}^C Y_{11}^C+ X_{22}^S Y_{11}^S).
\end{gather*} 
These two equations from $C_b^1$ prescribe the form of the harmonics of $Y_2$, leaving $Y_{20}$ as an undetermined free function of $\phi$ at this point. 

\paragraph{Higher order $\epsilon^n$}: let us now see how these constructions for the lower orders generalise for arbitrarily high order expansion $n$. Let us start with the set of $\kappa_0$ and $\tau_0$ equations that we generally refer to by $C_\perp^n$. \par
Following the steps taken for the lower orders, we would like to generalise a procedure to obtain an explicit close form for $Z_{n+1}$. The equations we are concerned with are order $\epsilon^n$, while the $Z$ functions of interest is an order higher. That means that only terms that include flux partial derivatives and $Z$ will possibly contribute. Furthermore, the relevant termsshould not have additional factors that will reduce the order of $Z$ (e.g. factors of $B_{\theta}$). \par
Looking at the $Z_{n+1}$ terms,
\begin{gather*}
    C_\kappa^n:~~~~~~~-B_{\alpha0}\left[\Bar{Y}_1\frac{n+1}{2}Z_{n+1,m}-m\Bar{Z}_{n+1,m}\frac{1}{2}Y_1\right]=\dots \\
    C_\tau^n:~~~~~~~~-B_{\alpha0}\left[-\Bar{X}_1\frac{n+1}{2}Z_{n+1,m}+m\Bar{Z}_{n+1,m}\frac{1}{2}X_1\right]=\dots
\end{gather*} 
where the dots represent terms other than $Z_{n+1}$ and the barred functions suggest interchange of the sine and cosine coefficients with a change of sign to the cosine term (as a result of a $\chi$ derivative). All the terms in the dots are necessarily of lower order than $n+1$ given that $B_{\theta0}$, $B_{\theta1}$ and $Z_1$ are all zero. With this observation, it is straightforward to show that the correct construction, to any order, to obtain a closed form for $Z_{n+1}$ consists of adding $X_1 C_\kappa^n+Y_1 C_\tau^n$, from which,
\begin{equation*}
    B_{\alpha0}\sqrt{B_0}(n+1)Z_{n+1,m}=\dots
\end{equation*}
We also saw in the lower orders of the expansion that the $C_\perp$ equations seemed to constraint the largest harmonics of $B_{\theta n}$ to vanish. We may show that this will in fact be true at all orders indeed. To oder $\epsilon^n$, the largest harmonic in the equations is $n+2$, which therefore leads to $n+3$ component constraints associated to each $C_\kappa^n$ and $C_\tau^n$. Let us see what the largest harmonic looks like for (\ref{eq:Ck}) and (\ref{eq:Ct}). Take $C_\kappa^n$ as an example, it is clear that the only possible contributions will come from, again, terms with partial $\psi$ derivatives, and in particular
\begin{equation*}
    -B_{\alpha0}\sum_{m=1}^{n-1}(\partial_\chi Y_{n+1-m}\partial_\psi Z_m-\partial_\chi Z_m\partial_\psi Y_{n+1-m})-B_{\theta n+1}\partial_\psi Y_1\frac{\mathrm{d}l}{\mathrm{d}\phi}
\end{equation*} 
Now, we are interested in the largest harmonic possible, which requires \textit{saturation} of each of the functions; i.e., if a function appears at an order $m$, then we must consider the $m$-th harmonic coefficient for it (this sefinition of \textit{saturation} will be employed again later). Otherwise, it would not contribute to the largest harmonic. Let us see what the implications of this are in the `commutation term' that appears in the summation in the expression above. Consider some $m$,
\begin{align*}
    \partial_\chi& Y_{n+1-m}\partial_\psi Z_m-\partial_chi Z_{n+1-m}\partial_\psi Y_m=\\
    &=\frac{m(n+1-m)}{2}\left(\bar{Y}_{n+1-m}Z_m-\bar{Z}_mY_{n+1-m}\right)=\\
    &\propto\left[\cos(n+1)\chi\left(Y_{n+1-m}^SZ_m^C+Y_{n+1-m}^CZ_m^S-Y_{n+1-m}^CZ_m^S-Y_{n+1-m}^SZ_m^C\right)+\right.\\
    &\left.+\sin(n+1)\chi\dots\right]
\end{align*}
where we used $\cos a\cos b=[\cos(a+b)+\cos(a-b)]/2$ and similar multiple angle formulas to obtain the relevant $n+2$ harmonics. These commutation terms vanish exactly, and therefore the only contribution to the $n+2$ harmonic comes from the $B_{\theta n+1}$ term. In particular, we get
\begin{gather*}
    -B_{\theta n+1,n+1}\partial_\psi Y_1\frac{\mathrm{d}l}{\mathrm{d}\phi}=0 \\
    B_{\theta n+1,n+1}\partial_\psi X_1\frac{\mathrm{d}l}{\mathrm{d}\phi}=0
\end{gather*}
And thus,
\begin{equation}
    B_{\theta n+1,n+1}=0.
\end{equation}
It is important to note that, this trivial solution takes in fact the place of four constraint equations (corresponidng to the largest harmonic of both $C_\kappa$ and $C_\tau$). Just as a quick recounting of what we have so far found: of the $2(n+3)$ constraint equations available from $C_\perp^n$, 4 of them lead to the vanishing of the largest harmonic of $B_\theta$, while $n+2$ constraints go into $Z_{n+1}$. Thus, a total of $n$ constraint equations are left. \par
For this $n$ remaining equations, we shall invoke the alternative form of the equations (\ref{eq:alterC1}) and (\ref{eq:alterC2}). As a matter of fact, we would like to obtain $n$ equations that would account for those $n$ degrees of freedom left, and which would not involve any explicit reference to the $Z_{n+1}$ we have already solved for using parts of $C_\perp^n$. Let us look at leading order forms of the equations (order $\epsilon^{n-1}$ for the $B_\psi$ and $\epsilon^{n+1}$ for the $B_\theta$), which we may write,
\begin{gather*}
    B_{\theta n+1,m}B_{\alpha0}B_0=m\frac{\mathrm{d}l}{\mathrm{d}\phi}\Bar{Z}_{n+1,m}+\dots \\
    B_{\psi n-1,m}B_{\alpha0}B_0=\frac{n+1}{2}\frac{\mathrm{d}l}{\mathrm{d}\phi}Z_{n+1,m}+\dots
\end{gather*}
where, again, the dots represent lower order terms. It is a straightforward operation to eliminate the $Z_{n+1,m}$ terms, and to write,
\begin{gather}
    B_{\theta n+1,m}^C=\frac{2m}{n+1}B_{\psi n-1,m}^S+\dots \label{eq:CpBpSBtC}\\
    B_{\theta n+1,m}^S=-\frac{2m}{n+1}B_{\psi n-1,m}^C+\dots \label{eq:CpBpCBtS}
\end{gather}
with $m=n-1,n-3\dots\in\mathbb{N}$. As wanted, these constitute in fact $n$ constraint equations which relate functions $B_\psi$ to $B_\theta$ and other lower order functions. An account of the relevant functions can be done by looking at the original equation. This shows that we may express $B_{\psi n-1}$ in terms of $B_{\theta n+1},~B_{\psi n-2},~X_{n},~Y_{n}$ and $Z_{n}$. \par
It is important to have a special consideration for the $m=0$ case. The same way as it resulted convenient when we looked at order $\epsilon^1$, the $m=0$ equation should be taken as a differential equation for $Y_{n}$ for higher orders as well. This will occur every other order (when the order of expansion is even), and in fact leaves $B_{\psi n 0}$ functions undetermined. It is important to enphasise that a differential equation needs to be solved here, as opposed to the algebraic solutions that we were able to construct previously and in what follows. The periodic condition will serve as boundary condition. Futhermore, the resultant equation depends on $B_{\theta n0}$ only, and no other form of $B_\theta$ directily, as it is clear from the equation (\ref{eq:alterC2}).    \par
It could be objected that we have in fact not made use solely of the $C_\perp$, as we have in fact used the alternative form of the equations (\ref{eq:alterC1}) and (\ref{eq:alterC2}). This is technically true: the equations constitute different projections, and as such, alternative linear combinations of the equations.  independent of the degrees of freedom already used, and in fact involving functions . Alternatively, one could consider taking the $Z_{n+1}$ form constructed explicitly and substitute it back into one of the equations of the $C_\perp$ set. This procedure is however significantly more convoluted. \par
Proceeding in the same way as for the Jacobian equations, we represent these $C_\perp$ equations diagramatically. Note that the complexity of the diagram is quite more involved than in the $J^n$ case, both because of having effectively two equations (two vector components instead of a scalar one) and the distinction between odd and even orders. See Fig. \ref{fig:CperpeqDiag} for the details.
\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{figures/Chapter3/CperpeqDiag.jpg}
    \caption{\textbf{Diagram for the $C_\perp^n$ equations.} The green shaded circle represents the function that one should solve the equation for ($B_{\psi n-1},~Z_{n+1}$). In this case, $Y_n$ has been shaded reddish to indicate that every other order, one should in fact solve for one of the components of $Y$ as well. The blue shade represents the fact that the $B_{\psi n0}$ functions are a priori not pinned down by the equations. The arrows indicate the leading order of the functions needed to find a solution (with broken lines representing the only even order case).}
    \label{fig:CperpeqDiag}
\end{figure}
\par
Having dealt with $C_\perp^n$, we should now turn our attention to the $C_b^n$ equation. This $\hat{\n{b}}_0$ component of the equation has $n+1$ harmonic components, and thus $n+1$ independent constraint equations. These shall be used to solve for $Y_{n+1}$ much in tehe fashion we showed explicitly in the first few orders. To show this to be the case, we could consider the $n$-th order form of $C_b^n$, focusing on the $Y_{n+1}$ coefficient, and tracking the largest order of the remaining functions. Doing so, we may write,
\begin{equation}
    -\frac{B_{\alpha0}}{2}\left[\Bar{X}_1(n+1)Y_{n+1}-mX_1\Bar{Y}_{n+1,m}\right]=\dots,
\end{equation}
where the dots represent some combination of functions $B_{\psi n-2},~X_{n+1},~B_{\theta n}$ and $Z_n$. It is also to be considered that $C_b^n$ has $n+1$ harmonic constraints in it. This is true because any possible $n+2$ harmonic must come from either the first commuting term or the $B_\theta$ piece, and both these contributions vanish: the first from the commutation when saturated Fourier coefficients are considered, and the second from the vanishing of the saturated coefficients of $B_\theta$. \par
Thus the constraint equations are enough to pin down $n+1$ of the $n+2$ components of $Y_{n+1}$. One could ask: what happens with the unconstraint remaining functions? Well, we have said in the preceeding that, every other order, one of the $C_\perp$ constraints should be employed to constraint $Y$, and thus that eliminates one of the degrees of freedom. The other one, however, truly manifests as an unconstraint function, and will only come to being further constraint when force balance is considered. This free function corresponds to the $Y_{n0}$ at every even order, representing the free addition of a flux function to the function $Y$. Again, we summarise these findings in a diagram (see Fig. \ref{fig:CbeqDiag}).
\begin{figure}
    \centering
    \includegraphics[width=0.65\textwidth]{figures/Chapter3/CbeqDiag.jpg}
    \caption{\textbf{Diagram for the $C_b^n$ equation.} The green shaded circle represents the function that one should solve the equation for ($Y_n$). The blue shade represents the fact that the $Y_{n0}$ functions are a priori not pinned down by the equations. The arrows indicate the leading order of the functions needed to find a solution.}
    \label{fig:CbeqDiag}
\end{figure}

\subsubsection{Summary magnetic construction}
As a brief summary, and re-counting the functions and constraint equations at our disposal, we present Table \ref{tab:countingQSJCaxis}. Thus this magnetic construction allows to determine $X$ and $Z$, as well as $B_\psi$ and $Y$ up to a flux function, constrianing some of the components of $B_\theta$, which is otherwise free. Every other order a differential equation needs to be solved. \par
The total counting will be again explored when specific considerations for the force balance are adopted. Then, we will be in a place to discuss the construction of solutions fully. 

\begin{table}[]
    \centering \hspace*{-.5cm}
    \begin{tabular}{|c||c|c|c|c|}
        \hline
    Eqn. & Order & Solve for\dots & in terms of\dots & Nb. eqns \\ \hline\hline
    $J^n$ & $n$ & $X_n$ & $Z_n, Y_{n-1},X_{n-1}$ & $n+1$ \\\hline
    $C_b^n$ & $n$ & $Y_{n+1}$ & $B_{\theta n},B_{\psi n-2}$ & \\
     & & & $Z_n, Y_{n},X_{n+1}$ & $n+1$ \\\hline 
    $C_\perp^n$ & $n=2k$ & $B_{\psi n-1}$ & $B_{\theta n+1},B_{\psi n-2}$ &  \\ 
    & & & $Z_{n}, Y_{n},X_{n}$ & $n$ \\
     &  & $Z_{n+1}$ & $B_{\theta n},B_{\psi n-1}$ &  \\
     & & & $Z_{n}, Y_{n},X_{n}$ & $n+2$ \\
     &  & $B_{\theta n+1,n+1}$ & 0 & $2*$ \\ \hline
    $C_\perp^n$ & $n=2k+1$ & $Y_n$ & $B_{\theta n+1,0}(\mathrm{only}),B_{\psi n-2}$ &  \\
    & & & $Z_{n-1}, Y_{n-1},X_{n-1}$ & $1"$ \\
     &   & $B_{\psi n-1}$ & $B_{\theta n+1},B_{\psi n-2}$ & \\
     & & & $Z_{n}, Y_{n},X_{n}$ & $n-1$ \\
     &   & $Z_{n+1}$ & $B_{\theta n},B_{\psi n-1}$ & \\
     & & & $Z_{n}, Y_{n},X_{n}$ & $n+2$ \\
     &   & $B_{\theta n+1,n+1}$ & 0 & $2*$ \\\hline
    \end{tabular}
    \caption{Counting of equations and degrees of freedom. each column shows: the label of equations, the order of expansion, what the equations are solved for, in terms of what other functions they are expressed, and the number of consraints (or independent equations) they amount to. The asterisk indicates that due to a trivial solution, two other consteraints are also satisfied by the trivial solution (but we drop them so that the total counting can be done correctly). The " indicates that a differential equation needs to be solved subject to periodic boundary conditions, unlike the rest of equations which simply require algebraic manipulations.}
    \label{tab:countingQSJCaxis}
\end{table}

\section{Near-axis expansion with force-balance: magnetostatic equilibrium} \label{NAEMS}
This section should not report findings other than those obtained by the procedure sketched by \cite{garrenboozer1991b}. It is nevertheless the basic equilibrium force balance to check the more general construction presented in the previous section. \par
In doing so, we shall learn in what way this particular force balance,
\begin{equation*}
    \n{j}\times\n{B}=\nabla p,
\end{equation*}
modifies the construction. With such a scalar pressure, we know beforehand that the the problem is quite significantly simplified, as it is manifest by the existence of Boozer coordinates. Another simplifying aspect is that the pressure is actually a flux function as a result of the form of the force balance. However, in preparation for the more general case, we shall not take these considerations as given, but merely obtained them from the ordered analysis of the equations.

\subsection{Constructing force balance equations}
In order to bring our magnetics construction of the previous section in contact with the magnetostatic force balance, we need to write the latter in a convenient way. For once, we should express all terms involving the magnetic field $\n{B}$ in terms of either the known covariant or contravariant forms. And once done, the vector equation needs to be projected along three independent directions. Let us start with the first consideration. \par
What form of the magnetic field shall we choose? The guiding principle that we shall abide by is to try to make equations as clear and as uncluttered as possible, possibly including a minimal number of functions. The first step is natural: to compute the current $\n{j}$ as $\nabla\times\n{B}$, one should use the covariant form of the magnetic field to write,
\begin{align}
    \n{j}=\left(\partial_\psi B_\theta-\partial_\chi B_\psi\right)J^{-1}\frac{\partial\n{x}}{\partial\phi}+\left(\partial_\chi B_\alpha-\Bar{\iota}\partial_\chi B_\theta-\partial_\phi B_\theta\right)J^{-1}\frac{\partial\n{x}}{\partial\psi}+\nonumber\\
    +\left[\partial_\phi B_\psi-\partial_\psi B_\alpha +\partial_\psi(\Bar{\iota}B_\theta)\right]J^{-1}\frac{\partial\n{x}}{\partial\chi} 
\end{align}
where we have made use of the dual relations and $J$ is as usual the Jacobian associated to our Boozer-like coordinate system. Now we need to cross the current density with the magnetic field $\n{B}$. Given the orthonormal relations of the $\partial\n{x}/\partial q$ and $\nabla q$ sets, it is now most natural to use the contravariant form of he magnetic field, to yield
\begin{align}
    \n{j}\times\n{B}=-J^{-1}\left\{\Bar{\iota}\left(\partial_\psi B_\theta-\partial_\chi B_\psi\right)-\left[\partial_\phi B_\psi-\partial_\psi B_\alpha +\partial_\psi(\Bar{\iota}B_\theta)\right]\right\}\nabla\psi-\nonumber\\
    -J^{-1}\left(\partial_\chi B_\alpha-\Bar{\iota}\partial_\chi B_\theta-\partial_\phi B_\theta\right)(\Bar{\iota}\nabla\phi-\nabla\chi). \label{eq:lhsFBal}
\end{align}
Given that we have now the LHS of the force balance equation written in the way shown, we may write,
\begin{equation}
    \nabla p=\partial_\psi p\nabla\psi+\partial_\chi p \nabla\chi+\partial_\phi p\nabla\phi.\label{eq:rhsFB}
\end{equation}
With no explicit reference to $\n{B}$ left, we may now move on to obtaining the three independent components of the vector equation that form (\ref{eq:lhsFBal}) and (\ref{eq:rhsFB}). Again, the most natural choice seems to be the set $\{\nabla\psi,\nabla\chi,\nabla\phi\}$, which by construction have a non-zero Jacobian everywhere, and thus form a valid basis. Thus, we may simply read out the equations,
\begin{gather}
    \mathrm{III}:~~~~~~~~\Bar{\iota}\left(\partial_\psi B_\theta-\partial_\chi B_\psi\right)-\left[\partial_\phi B_\psi-\partial_\psi B_\alpha +\partial_\psi(\Bar{\iota}B_\theta)\right]+J\partial_\psi p=0 \\
    -\Bar{\iota}\left(\Bar{\iota}\partial_\chi B_\theta+\partial_\phi B_\theta\right)+J\partial_\phi p=0 \nonumber \\
    \mathrm{II}:~~~~~~~~ \Bar{\iota}\partial_\chi B_\theta+\partial_\phi B_\theta-J\partial_\chi p=0.
\end{gather}
where we have used the fact that $B_\alpha=B_\alpha(\psi)$ in our construction. We have not labelled the second of the equations, because it may be almost trivially combined with the latter to yield,
\begin{equation}
    \mathrm{I}:~~~~~~~~(\partial_\phi+\Bar{\iota}\partial_\chi)p=0. \label{eq:b.gP0}
\end{equation}
Note that this latter equation is in fact $\n{B}\cdot\nabla p =0$, and in fact, we shall see that its implications are as expected.

\subsection{Expansion procedure: magnetostatic force balance}
Let us take the equations just introduced one by one, and proceed order by order as we did in the case of the nmagnetic equations.
\subsubsection{Equation I}
As advertised, equation I is nothing but $\n{B}\cdot\nabla p=0$, and thus we expect the solution to the equation to be that $p=p(\psi)$. Let us see how this shows up order by order.
\paragraph{Order $\epsilon^0$:} 
\begin{equation*}
    \partial_\phi p_0=0 \rightarrow p_0=\mathrm{const.}
\end{equation*}

\paragraph{Order $\epsilon^1$:}
\begin{gather*}
    p_{11}^C{}'+\Bar{\iota}_0p_{11}^S=0 \\
    p_{11}^S{}'-\Bar{\iota}_0p_{11}^C=0
\end{gather*}
We may substitute one into another to obtain a SHO equation,
\begin{equation*}
    \left(p_{11}^C\right)''+\Bar{\iota}_0^2 p_{11}^C=0.
\end{equation*}
The solution to such an equation will be oscillating with $\phi$ and frequency $\Bar{\iota}_0$, $p_{11}^C\sim\exp(\pm i\Bar{\iota}_0\phi)$. Now, for a rotational transform that is generally irrational, it is clear that the solution to this equation will not be periodic in $\phi$ (meaning that $p_{11}^C(0)\neq p_{11}^C(2\pi)$). As $p$ is a physically meaningful quantity it must be periodic in the angular coordinates, as otherwise would be multivalued. This physicality requirement forces the solution to be trivial. I.e.,
\begin{equation*}
    p_{11}^C=0=p_{11}^S
\end{equation*}

\paragraph{Higher order:} an identical argument to that for $O(\epsilon^1)$ holds for arbitrarily large order. Just for completeness, we may write,
\begin{gather*}
    p_{nm}^C{}'+m\Bar{\iota}_0p_{nm}^S=0 \\
    p_{nm}^S{}'-m\Bar{\iota}_0p_{nm}^C=0,
\end{gather*}
from which by analogy it follows that $p_{nm}^C=0=p_{11}^S$. For the $p_{n0}$ term, the corresponding equation simply forces it to be a constant. Altogether, we recover the advertised consequence that order by order, the pressure function is forced into being a flux function,
\begin{equation}
    p=p(\psi).
\end{equation}

\subsubsection{Equation II:} let us now focus order by order on,
\begin{equation*}
    \Bar{\iota}\partial_\chi B_\theta+\partial_\phi B_\theta=0,
\end{equation*}
where we have already put into use the fact that the pressure is a flux function as shown from Equation I. The equation we obtain is identical in form to that of equation I, but this time the magnetic equation is on $B_\theta$. \par
We shall spare ourselves from repeating the process in an identical way as we did before, and thus we shall simply write that $B_\theta=B_\theta(\psi)$. So we see that the form of $B_\theta$ is pinned down by the force balance up to constant coefficients. This view is consistent to the treatment we gave to $B_\theta$ in the magnetic equations, in which we did not solve for $B_\theta$ at any point. Imprtantly, the magnetics and force balance are clearly interconnected by this covariant function.

\subsubsection{Equation III}: finally, we have 
\begin{equation*}
    \Bar{\iota}\left(\partial_\psi B_\theta-\partial_\chi B_\psi\right)-\left[\partial_\phi B_\psi-\partial_\psi B_\alpha +\partial_\psi(\Bar{\iota}B_\theta)\right]+J\partial_\psi p=0
\end{equation*}
This equation could be regarded as one for $B_\psi$ expressed in terms of the pressure and the magnetic field strength. This is the standard equation relating $B_\psi$ to the force balance, and specifying the angular dependence of the function to be equal to that of $1/B^2$. One would indeed obtain the same result in the standard way (without expansion), by taking a flux surface average and subtracting it from the original equation. \par
However, let us see how this comes to play in our expansion approach. 

\paragraph{Order $\epsilon^0$}: 
\begin{equation*}
    -B_{\psi0}'+B_{\alpha1}+B_{\alpha0}B_0 p_{20}=0
\end{equation*}
from which it follows that $B_{\psi0}=\mathrm{const.}$, and we obtain an additional condition, this time relating constant coefficients,
\begin{equation*}
    B_0p_{20}=-\frac{B_{\alpha1}}{B_{\alpha0}}.
\end{equation*}

\paragraph{Order $\epsilon^1$}: 
\begin{gather*}
    \Bar{\iota}_0B_{\psi11}^S-B_{\alpha0}B_{11}^C p_{20}+B_{\psi11}^C{}'=0 \\
    \Bar{\iota}_0 B_{\psi11}^C=B_{\psi11}^S{}'
\end{gather*}
This is again a set of equations that when combined gives respective SHO equations for the $B_\psi$ components. From the requirement of periodicity, the general solution must be taken to be trivial (as the `oscillation' is generally irrational), and thus we are concerned only with the particular solution. Thus,
\begin{gather*}
    B_{\psi11}^S=\frac{B_{\alpha0}}{\Bar{\iota}_0}B_{11}^C p_{20} \\
    B_{\psi11}^C=0
\end{gather*} 
Note that the coefficients of $B_\psi$ end up being constant, and not more general functions of $\phi$, which implies that $B_\psi$ shares the same angular dependence as $1/B^2$. This is precisely what we expected.

\paragraph{Higher order}: we shall spare ourselves from a general expression for the equations that one would obtain by looking at higher orders of the expansion. However, we shall remark the structure of the equations. The set may be understood as defining the function $B_\psi$ to the $n$-th order. That constitutes $n+1$ constraints to order $\epsilon^n$. 

\subsubsection{Summary magnetostatic construction} We have seen from the magnetostatic force balance that we obtain three sets of constraint, summarised in Table
\ref{tab:countingQSMSaxis}.

\begin{table}[H]
    \centering \hspace*{-.5cm}
    \begin{tabular}{|c||c|c|c|c|}
        \hline
    Eqn. & Order & Solve for\dots & in terms of\dots & Nb. eqns \\ \hline\hline
    I & $n$ & $p_n$ & const.$|0$ & $n+1$ \\\hline
    II & $n$ & $B_{\theta n}$ & const.$|0$ & $n+1$ \\\hline 
    III & $n$ & $B_{\psi n}$ & const. & $n+1$ \\\hline
    \end{tabular}
    \caption{Counting of equations and degrees of freedom. each column shows: the label of equations, the order of expansion, what the equations are solved for, in terms of what other functions they are expressed, and the number of consraints (or independent equations) they amount to. Note that in the magnetostatic case the dependency of the equations mostly results in constants.}
    \label{tab:countingQSMSaxis}
\end{table}

\subsection{Complete magnetostatic equilibrium near-axis construction}
Once that we have separatedly explored the equations for force balance (this section \ref{NAEMS}) and the purely magnetic considerations (in section \ref{NAEmagn}), it is time to bring them together and delve into how would one construct solutions for this expansion procedure. \par
For that, we shall make use of the information in Tables \ref{tab:countingQSJCaxis} and \ref{tab:countingQSMSaxis}, which will be vital for counting the number of equations and available degrees of freedom. Given the dimensions of the problem, we must develop an efficient way of doing this counting and construction in an orderly manner. A way that will ultimately be applied to more complicated forms of force balance. \par
First, we should know to a given order how do the different functions come into play. The question that needs to be addressed is: how can we add higher orders of the expansion in such a way that the problem formulated is self consistent? The answer is shown in Fig. \ref{fig:ConstructNAMS}. \par
\begin{figure}
    \hspace*{+0.5cm}\includegraphics[width=0.8\textwidth]{figures/Chapter3/MSfunOrder.jpg}
    \caption{\textbf{Consistent order of functions.} Order of functions that ought to be simultaneously solved for. The color code represents: green - precise constraint number for the number of functions, blue - additional free functions every even order, orange - additional constraints.}
    \label{fig:ConstructNAMS}
\end{figure}
Secondly, we should indicate which equations are to be solved to determine which functions and to what order: i.e, how are we going to construct the solution. This collection is shown in Table \ref{tab:countingQSMSaxis}. \par
\begin{table}[]
    \centering \hspace*{-.5cm}
    \begin{tabular}{c|c|c|c|c|c|c|}
    MS & $X_n$ & $Y_n$ & $Z_n$ & $B_{\theta n}$ & $B_{\psi n}$ & $p_n$ \\ \hline\hline
    0 &  \cellcolor{black} & \cellcolor{black} & \cellcolor{black} &  & \small III$^0$ &   \\\cline{2-4}\cline{6-6}
    1 & $J^1$ & \tiny $C_b^0$|$\tilde{C}_\perp^1(1)$ & $C_\perp^0$ & II & \tiny \cellcolor{Apricot} $C_\perp^2(2)$|III$^1(2)$ & I  \\\cline{2-4}\cline{6-6} 
    2 &  $J^2$ & \tiny\cellcolor{CornflowerBlue} $C_b^1(2)$|$Y_{20}$ & $C_\perp^1$ & \tiny $(\psi)$ &  \tiny \cellcolor{Apricot} $C_\perp^3(2)$|III$^2(3)$  & \tiny $(\psi)$  \\\cline{2-4}\cline{6-6}
    3 &  $J^3$ & \tiny $C_b^2$|$\tilde{C}_\perp^3(1)$  & $C_\perp^2$ &  & \tiny \cellcolor{Apricot} $C_\perp^4(4)$|III$^3(4)$ &  \\\hline
    \end{tabular}
    \caption{\textbf{Magnetostatic near-axis construction,} Each cell represents the equations that need to be solved to find a function (column) at a given order (row). The equation labels are the ones introduced in the text: $J$ for the Jacobian equation, $C_\perp$ and $C_b$ for the co(ntra)variant perpendicular and $b_0$ components, and I, II and III for the force balance equations. The numbers in parenthesis denote the number of constraint equations (where no number is given is because they account for the precise number of unknowns in that cell). The undivided 4th and last columns represent the fact that the functions are flux functions. The blue color shows that a new free function is being introduced, while the light orange represents an overconstraint (multiple equations for the same function). }
    \label{tab:eqConstructNAMS}
\end{table}
With these two tools in our hands, we are now in a position to perform the counting in an effective way. As observed in \cite{garrenboozer1991b}, it is evident that the problem is overconstraint. The heart of the problem lies on $B_\psi$, a function that is both determined by the magnetic equations as well as the force balance one (orange colored equations). This overdetermination translates into additional constraint equations involving the other functions at the relevant order and lower. Generally, this implies an overconstraint problem, given that we already have (as shown in Tab. \ref{tab:eqConstructNAMS}) indepoendent ways of constructing those functions. By doing this counting, we see that at a given order $n$, and thus for $B_{\psi n-1}$ (see Fig. \ref{fig:ConstructNAMS}), we have $n$ or $n-1$ (depending on whether the order is even or odd) extra constraints. For a completely correct counting, we should take into account the extra free functions that at every other order comes from $Y_{n0}$. Addig these two bits together, a total of $n-1$ over-constrianing equations appear at each order. \par
Thus, in the magnetostatic limit, we arrive at the same conclusions as previously shown in \cite{garrenboozer1991b}. To the lowest order ($n=1$), there is a straightforward solution to the near-axis quasisymmetric field, as there is no overconstraining equation. However, to second order ($n=2$), the construction of the solution is not so simple. \par
First of all because we do in principle have one overconstraining equation. To satisfy such an equation, one is forced to relax the free nature of the magnetic axis. Infact, the only functions that are left unpinned are the axis curvature $\kappa$ and torsion $\tau$. The overconstraining equations left will then constriant one of these functions. \par
In practice, we should take the magnetic equations describing $B_{\psi11}$, and substitute the closed forms obtained from the force balance equation III. These shall constitute two differential equations that are to be solved for $Y_{20}$ and $\kappa$ for instance. \todo{Need to write down explicitly, but note that it is quite a mess.}
 

\section{Near-axis expansion with force-balance: anisotropic pressure} \label{NAEMS}

We saw in the previous section how the magnetostatic equilibrium breaks the expansion for the magnetic field close to the magnetic axis to the third order. This overdetermination prevents the expansion to be carried to higher orders, and thus suggests that there is no way in which a globally quasisymmetric field might be constructed (at least not in this way). \par
However, formally speaking, there is no reason why one should stick to the magnetostatic equilibrium case, which seems to be the source of trouble. A natural hypothesis is that by introducing a more general form of force balance, which might include additional degrees of freedom, the overdetermination problem will cease. This is because there does not seem to be any fundamental break-down of the expansion-construction other than us having too little freedom. \par
In this section we shall be concerned with the pjhysically meaningful problem of anisotropic pressure. Including a pressure tensor is the most immediate and natural extension to the magnetostatic equilibrium (which is a special case).

\subsection{Constructing force balance equations}
To incorporate the anisotropic force balance to the near-axis construction, we should cast it in a manageable and useful way. Here we shall mimic to as much an extent as possible the procedure we followed in the magnetostatic case. \par
Let us begin by writing down the force balance,
\begin{equation}
    \n{j}\times\n{B}=\nabla\cdot\Pi,
\end{equation}
where,
\begin{equation}
    \Pi=(p_\parallel-p_\perp)\n{b}\n{b}+p_\perp \mathbb{I}.
\end{equation}
The unit diad is given by $\mathbb{I}$, $p_\parallel$ represents the pressure along the field line and $p_\perp$ that perpendicular to them. Note hoe, in the ispotropic limit that $p_\parallel=p_\perp$, one recovers the isotropic magnetostatic force balance. \par
In order to write down any useful form, we need to explicitly take the divergence of the pressure tensor $\Pi$. Because most of our knowledge of the magnetic field is based on $\n{B}$ rather than its associated unit vector, we shall favour the former and write
\begin{align*}
    \nabla\cdot\Pi=&\nabla\cdot\Bigl[\underbrace{\frac{p_\parallel-p_\perp}{B^2}}_{\Delta}\n{B}\n{B}+p_\perp\mathbb{I}\Bigr]=\nabla  p_\perp +(\n{B}\cdot\nabla\Delta) \n{B}+\Delta \n{B}\cdot\nabla\n{B}=\\
    =&\nabla  p_\perp +(\n{B}\cdot\nabla\Delta) \n{B}+\Delta \nabla\left(\frac{B^2}{2}\right)+\Delta\n{j}\times\n{B},
\end{align*}
where for the latter we used $\n{B}\cdot\nabla\n{B}=\nabla(B^2/2)+\n{j}\times\n{B}$. Thus, we may rewrite the force balance equation in the form,
\begin{equation}
    (1-\Delta)\n{j}\times\n{B}=(\n{B}\cdot\nabla\Delta) \n{B}+\Delta\nabla\left(\frac{B^2}{2}\right)+\nabla p_\perp
\end{equation}
For the LHS, we shall use the form previously found for $\n{j}\times\n{B}$ in (\ref{eq:lhsFBal}),
\begin{equation*}
    \n{j}\times\n{B}=(-\Bar{\iota}A_\alpha\nabla\phi-A_\psi\nabla\psi+A_\alpha\nabla\chi)J^{-1}
\end{equation*}
where,
\begin{gather*}
    A_\alpha=(\partial_\phi+\Bar{\iota}\partial_\chi)B_\theta \\
    A_\psi=\partial_\psi B_\alpha-(\partial_\phi+\Bar{\iota}\partial_\chi)B_\psi-B_\theta\Bar{\iota}',
\end{gather*}
and $\Bar{\iota}'=\partial_\psi\Bar{\iota}$. \par
Because of the functions we chose to expand, we should also modify the gradient $\nabla(B^2/2)$ to make it act on the more convenient $1/B^2$. For such purpose,
\begin{equation*}
    -\nabla\left(\frac{B^2}{2}\right)=\frac{1}{2}B^4\nabla\left(\frac{1}{B^2}\right)=\frac{1}{2}J^{-2}B_\alpha^2\nabla\left(\frac{1}{B^2}\right).
\end{equation*} 
Finally we will have to use the covariant form for the explicit magnetic field vector in the equation, and the contravariant form for the magnetic equations $\n{B}\cdot\nabla\dots=J^{-1}(\partial_\phi+\Bar{\iota}\partial_\chi)\dots$. With all of this rewriting of the equations, we write the three relevant components of the equation by reading out the factors of the basis $\{\nabla\psi,\nabla\chi,\nabla\phi\}$.
\begin{gather*}
    \nabla\phi:~~~\Bar{\iota}A_\alpha(1-\Delta)+(B_\alpha-\Bar{\iota}B_\theta)(\partial_\phi+\Bar{\iota}\partial_\chi)\Delta+J\partial_\phi p_\perp=0 \\
    \nabla\chi:~~~A_\alpha(1-\Delta)=B_\theta(\partial_\phi+\Bar{\iota}\partial_\chi)\Delta-\frac{1}{2}B_\alpha B^2\Delta\partial_\chi\left(\frac{1}{B^2}\right)+J\partial_\chi p_\perp=0 \\
    \nabla\psi:~~~A_\psi(1-\Delta)+B_\psi(\partial_\phi+\Bar{\iota}\partial_\chi)\Delta-\frac{1}{2}B_\alpha B^2\Delta\partial_\psi\left(\frac{1}{B^2}\right)+J\partial_\psi p_\perp=0.
\end{gather*}
The first two equations may be combined to obtain a simplified form without $A_\alpha$, and thus, our set of three force balance equations will be written as follows,
\begin{gather}
    \mathrm{I}:~~~\frac{1}{B^2}(\partial_\phi+\Bar{\iota}\partial_\chi)\Delta+\frac{1}{B^4}(\partial_\phi+\Bar{\iota}\partial_\chi)p_\perp=\frac{\Bar{\iota}}{2}\Delta\partial_\chi\left(\frac{1}{B^2}\right) \\
    \mathrm{II}:~~~A_\alpha(1-\Delta)=\frac{B_\theta}{B^2}\partial_\phi p_\perp +\frac{B_\alpha-\Bar{\iota}B_\theta}{B^2}\partial_\chi p_\perp-\frac{B_\alpha-\Bar{\iota}B_\theta}{2}B^2\Delta \partial_\chi\left(\frac{1}{B^2}\right) \\
    \mathrm{III}:~~~A_\psi(1-\Delta)+B_\psi(\partial_\phi+\Bar{\iota}\partial_\chi)\Delta-\frac{1}{2}B_\alpha B^2\Delta\partial_\psi\left(\frac{1}{B^2}\right)+J\partial_\psi p_\perp=0.
\end{gather}
Again, as we did in the magnetostatic case, we managed to express these force balance equations in a way that makes them be independent of the functions $X,~Y$ and $Z$, and thus only interact with the magnetic equations throught the functions $B_\theta$ and $B_\psi$, which will again be the centrestone of the construction.

\subsection{Expansion procedure: anisotropic force balance}
\subsubsection{Equation I}
It is quite noticeable the resemblence of this equation to that in the magnetostatic case. However the interpretation of the function that this set is to solved for will be slightly different.
\paragraph{Order $\epsilon^0$} 
\begin{equation*}
    B_0\partial_\phi p_{\perp0}+\partial_\phi\Delta_0=0
\end{equation*}
which simply gives,
\begin{equation}
    B_0 p_{0}+\Delta_0=\mathrm{const}
\end{equation}
So the angular dependence of the anisotropy must be on axis the same as that of the perpendicular oressure, with an undetermined overall level offset. Note that this allows in principle for $p_{\perp0}$ to be some periodic function of $\phi$, and tus not nbecessarily a flux function. In fact, this freedom seems to hold in the construction to any order.

\paragraph{Order $\epsilon^1$}
\begin{equation*}
    B_0(\partial_\phi+\Bar{\iota}\partial_\chi)(B_0 p_1+\Delta_1)=\frac{\Bar{\iota}}{2}\Delta_0\partial_\chi B_1+B_1\Delta_0'
\end{equation*}
where the prime denotes, as usual, a derivative with respect to $\phi$. Spelt out in terms of their harmonic coefficients, and taking $\Delta$ and $p_\perp$ both to have no particular symmetry to start with,
\begin{gather*}
    (B_0p_{11}^C+\Delta_{11}^C)'+\Bar{\iota}_0(B_0p_{11}^S+\Delta_{11}^S)=\frac{B_{11}^C}{B_0}\Delta_0' \\
    (B_0p_{11}^S+\Delta_{11}^S)'-\Bar{\iota}_0(B_0p_{11}^C+\Delta_{11}^C)=-\frac{\Bar{\iota}_0}{2}\frac{B_{11}^C}{B_0}\Delta_0.
\end{gather*} 
This structure should be reminescent of the magnetostatic case. Indeed, we may construct SHO equations associated to the harmonic components of the particular combination $B_0p_1+\Delta_1$. This way, one may write,
\begin{equation*}
    (B_0p_{11}^C+\Delta_{11}^C)''+\Bar{\iota}_0^2(B_0p_{11}^C+\Delta_{11}^C)=\frac{B_{11}^C}{B_0}\left(\frac{\Bar{\iota}_0^2}{2}\Delta_0+\Delta_0''\right)
\end{equation*}
where we took again the offset of the angular coordinates such that $B_{11}^S=0$.\par
Demanding periodicity on the pressure tensor amounts to necessarily dampiing the general solution of the equation. This is so, again, because of the general irrational nature of $\Bar{\iota}_0$, and the fact that the driving term (the RHS) is periodic. Thus, a solution to such a harmonic equation will correspond to a particular solution. \par
Given that we are dealing with periodic functions, it is natural to exploit Fourier tools to try and find the particular solution to the equation. Write,
\begin{equation*}
    \Delta_0=\sum_{n=0}^\infty\left(\Bar{\Delta}_{0n}^C\cos(n\phi)+\Bar{\Delta}_{0n}^S\sin(n\phi)\right).
\end{equation*}
and keep in mind that $\dots''=-n^2\dots$. Then, our harmonic equation gives
\begin{align}
    B_0p_{11}^C+\Delta_{11}^C&=-\eta\sum_{n=0}^\infty\frac{\Bar{\iota}_0^2-2n^2}{\Bar{\iota}_0^2-n^2}\left(\Bar{\Delta}_{0n}^S\sin n\phi+\Bar{\Delta}_{0n}^C\cos n\phi\right)
\end{align}
which is by construction periodic, and we have used the definition $\eta=-B_{11}^C/2B_0$. We may then also write,
\begin{equation}
    B_0p_{11}^S+\Delta_{11}^S=-\Bar{\iota}_0\eta\sum_{n=0}^\infty\frac{n}{\Bar{\iota}_0^2-n^2}\left(\Bar{\Delta}_{0n}^S\cos n\phi-\Bar{\Delta}_{0n}^C\sin n\phi\right). \label{eq:d11S}
\end{equation}
Interestingly, the sine component has a zero $\phi$ averaged value. \par
With this, we have again explicitly and successfully solved for $\Delta_{11}$ in terms of pressure and other lower order functions. \par

\paragraph{Higher order} To order $\epsilon^n$ the equations will have a similar structure as the one shown in the lower orders. In fact, to make this generalisation ever clearer, consider rewriting equation I slightly,
\begin{equation*}
    \frac{1}{B^2}(\partial_\phi+\Bar{\iota}\partial_\chi)\left(\Delta+\frac{p_\perp}{B^2}\right)=\frac{\Bar{\iota}}{2}\partial_\chi\left(\frac{1}{B^2}\right)\left[\frac{2 p_\perp}{B^2}+\Delta\right].
\end{equation*}
From this rewritten form, it is clear that the terms in this equation involving the largest expansion functions for a given order $n$ will have the structure,
\begin{equation*}
    B_0\left(\Delta_n+B_0 p_n\right)'+\Bar{\iota}_0B_0\partial_\chi\left(\Delta_n+B_0 p_n\right)=\dots,
\end{equation*}
where the dots represent combinations of lower order functions. \par
This structure to arbitrary order allows for a generalisation of the Fourier and SHO procedure employed for the lower orders explicitly shown. Thus, in fact, we may take our I equation to each order to determine $\Delta_n$ as a function of $p_n$ and lower order function, and thus consist of $n+1$ equations. \par
From this generalised form it is also clear that the $\Delta_{n0}$ function plays a very special role. In that case the equation is not a SHO one, but simply a first order ODE of the form $\partial_\phi f=g$. Though the solution is trivial to find, a periodic solution for $f$ will only exist provided that $\int g\mathrm{d}\phi=0$. This could in principle play the role of an additional constraint on the constant coefficients of the various functions.\par
We may very simply draw a diagram to represent this equation I to order $n$ as shown schematically in Fig. \ref{fig:aniIeqDiag}.
\begin{figure}
    \centering
    \includegraphics[width=0.25\textwidth]{figures/Chapter3/aniIeqDiag.jpg}
    \caption{\textbf{Diagram for equation I$^n$.} The green shaded circle represents the function that one should solve the equation for ($\Delta_n$). The arrows indicate the leading order of the functions needed to find a solution.}
    \label{fig:aniIeqDiag}
\end{figure}

To see how these general observations come into play, just for completeness we include the situation for I$^2$.

\paragraph{Order $\epsilon^2$} 
The non-harmonic term,
\begin{align*}
    (B_0p_{20}^C+\Delta_{20}^C)'&=-\frac{\Bar{\iota}_0}{4}\frac{B_{11}^C}{B_0}(4B_0p_{11}^S+3\Delta_{11}^S)+\frac{(B_{11}^C)^2\Delta_0'}{2B_0^2}+\frac{B_{20}^C}{B_0}\Delta_0'-\\ 
    &-\frac{B_{11}^C}{2B_0}(2B_0p_{11}^C+\Delta_{11}^C)'.
\end{align*}
Inspecting the RHS of the equation to see if the solubility condition is satisfied, it is evident that it will be subject to whether the first term has a vanishing $\phi$ average. This is so because all other terms are in fact derivatives. Having no more information regarding $p_{11}^S$ does make it impossible to determine whether it will vanish or not. However, we shall see later that $p_{11}^S=0$, and therefore, in conjuction with what we found from I$^1$, the solubility condition is satisfied. \todo{It is not clear whether this will generalise or not to higher orders}\par
The SHO-like part looks as expected,
\begin{gather*}
    \mathcal{A}+2\Bar{\iota}_0(BB_0p_{22}^S+\Delta_{22}^S)+(B_0p_{22}^C+\Delta_{22}^C)'=0\\
    \mathcal{B}-2\Bar{\iota}_0(BB_0p_{22}^C+\Delta_{22}^C)+(B_0p_{22}^S+\Delta_{22}^S)'=0.
\end{gather*}
Both $\mathcal{A}$ and $\mathcal{B}$ are a combination of lower order functions of $p$ and $\Delta$,
\begin{gather*}
    \mathcal{A}=\Bar{\iota}_0\left[-\frac{B_{22}^S}{B_0}\Delta_0+\frac{B_{11}^C}{4B_0}(4B_0p_{11}^S+\Delta_{11}^S)\right]-\frac{(B_{11}^C)^2}{2B_0^2}\Delta_0'-\frac{B_{22}^C}{B_0}\Delta_0'+\frac{B_{11}^C}{2B_0}(2B_0p_{11}^C+\Delta_{11}^C)'\\
    \mathcal{B}=\Bar{\iota}_0\left[\frac{B_{22}^C}{B_0}\Delta_0-\frac{B_{11}^C}{4B_0}(4B_0p_{11}^C+\Delta_{11}^C)\right]-\frac{B_{22}^S}{B_0}\Delta_0'+\frac{B_{11}^C}{2B_0}(2B_0p_{11}^S+\Delta_{11}^S)'.
\end{gather*}

\subsubsection{Equation II}
For this equation we shall skip the $\epsilon^0$ order, as the resultant equation is in fact a tautology that includes no more information other than what we already know. Thus, we should start off form the first order equation.
\paragraph{Order $\epsilon^1$}
To leading order,
\begin{equation*}
    \Delta_0\partial_\chi B_1-2B_0^2\partial_\chi p_1=0.
\end{equation*}
Considering the harmonics of the expression, we may write
\begin{gather*}
    B_0p_{11}^S=0 \\
    B_0p_{11}^C=-\eta\Delta_0.
\end{gather*}
Thus, the leading order gives closed form expressions for the first order pressure. The fact that the sine component of the pressure must vanish can be related to the particular choice of coordinate system, which we forced to be such that $B_{11}^S=0$. This piece of $p$ inherits such a choice.

\paragraph{Order $\epsilon^2$} 
The non-harmonic part of the equation is quite simple,
\begin{align*}
    \frac{\mathrm{d}}{\mathrm{d}\phi}\left[B_{\theta20}^C(1-\Delta_0)\right]=-\frac{B_{\alpha0}}{2}\eta\Delta_{11}^S
\end{align*}
and is easily checked to satisfy the solubility condition considering the form of $\Delta_{11}^S$ given in (\ref{eq:d11S}). In fact, we could go further and explicitly solved for $B_{\theta20}$ using the Fourier representation,
\begin{equation}
    B_{\theta20}^C(1-\Delta_0)=\Bar{B}_{\theta20}-B_{\alpha0}\frac{\Bar{\iota}_0\eta^2}{2}\sum_{n=0}^\infty\frac{1}{\Bar{\iota}_0^2-n^2}\left(\Bar{\Delta}_{0n}^S\sin n\phi+\Bar{\Delta}_{0n}^C\cos n\phi\right)
\end{equation}
where we have written $\Bar{B}_{\theta20}$ to represent the integration constant. \par
To this order, equation II yields two more equations corresponding to the $\cos2\chi$ and $\sin2\chi$ harmonics. This equation would involve $B_{\theta22}$ functions, and in fact would give a SH-like construction fo them. However, from our magnetic expansion we know that they must vanish, and thus the equations are to be understood in a different way. We shall not go into the details of these equations here, as we will show that, in any order, these equations are equivalent to part of the constraints in III. We will just say that the equations are in fact used to determine the form of $p$. 

\paragraph{Higher order} Let us now try to generalise our construction to any order $\epsilon^n$. To do so in an efficient way, we will rewrite equation II inspired by the behaviour at lowest orders,
\begin{equation}
    (\partial_\phi+\Bar{\iota}\partial_\chi)\left[B_\theta(1-\Delta)\right]=B_\alpha B^2\left[\frac{1}{B^4}\partial_\chi p_\perp-\frac{1}{2}\Delta\partial_\chi\left(\frac{1}{B^2}\right)\right].
\end{equation}
This is a very efficient way of writing equation II. It shows in a very clear way that to any order $\epsilon^n$, one may solve the equation for $B_{\theta n}$ in the LHS (and lower orders). The RHS will include $p_n$ and $\Delta_{n-1}$ in it. This constitutes a total amount of $n-1$ constraint equations, precisely the degrees of freedom in $B_{\theta n}$ (given  that we have shown to be a result of the magnetic equations that $B_{\theta nn}=0$). \par
If the solutions were to be constructed explicitly, as shown for the lower orders, we would have a SHO structure for the pairs $B_{\theta n m}^{C/S}$ for $0<m<n$, and a simple $\phi$ derivative for $B_{\theta n0}$. In that sense, the structure of the expanded equations is not dissimilar from that in equation I. Note that when $m=0$, we will not have $p_n$, but rather $p_{n-1}$ which will prove to be an important thing to note.  \par
A critical point in the way that we have counted the equations has been the dropping of the largest harmonic constraints (those that originally contained $B_{\theta nn}$). We claimed that one was allowed to drop these equations, because they were equivalent to those obtained from III for the highest harmonic. We now show that this is in fact the case for all $n$. \par
Let us compare,
\begin{gather*}
    \mathrm{II}:~~~A_\alpha(1-\Delta)=\frac{B_\theta}{B^2}\partial_\phi p_\perp +\frac{B_\alpha-\Bar{\iota}B_\theta}{B^2}\partial_\chi p_\perp-\frac{B_\alpha-\Bar{\iota}B_\theta}{2}B^2\Delta \partial_\chi\left(\frac{1}{B^2}\right) \\
    \mathrm{III}:~~~A_\psi(1-\Delta)+B_\psi(\partial_\phi+\Bar{\iota}\partial_\chi)\Delta-\frac{1}{2}B_\alpha B^2\Delta\partial_\psi\left(\frac{1}{B^2}\right)+J\partial_\psi p_\perp=0.
\end{gather*}
As we have said, we are concerned with the largest harmonic of the equations. In order to compare alikes, we shall look at order $\epsilon^n$ of II and $\epsilon^{n-2}$ of III, this difference being a consequence of the flux derivatives present in the latter. Again, if we are to construct the constraint equations associated to the largest possible harmonic, we shall consider only saturating terms of the Fourier expansion. I.e. if $p_n$ appears, then it will have to come as $p_{nn}$. This is so because $\cos k\sin l=[\sin(k+l)-\sin(k-l)]/2$. \par
With this saturating condition in mind, we may look at the terms that are relevant. For II,
\begin{equation*}
    -\frac{B_\alpha}{B^2}\partial_\chi p_\perp+\frac{B_\alpha}{2}B^2\Delta\partial_\chi\left(\frac{1}{B^2}\right)=0,
\end{equation*}
where all $B_\theta$ terms have been dropped, as $B_{\theta nn}=0$. \par
As for equation III, the somplifying logic is slightly different. The largest harmonics will possibly be achieved only by those terms that have $\psi$ derivatives, as they allow for for harmonics two orders higher than otherwise possible. Hence the considerations of III to $\epsilon^{n-2}$ compared to II. For III, the $\psi$ derivative terms read,
\begin{equation*}
    \partial_\psi B_\alpha(1-\Delta)-\frac{1}{2}B^2B_\alpha\Delta \partial_\psi\left(\frac{1}{B^2}\right)+\frac{B_\alpha}{B^2}\partial_\psi p_\perp=0.
\end{equation*}
When saturation of the functions is required, the following is true,
\begin{gather*}
    \partial_\psi f_{nn}=\frac{n}{2\epsilon^2}f_{nn} \\
    \partial_\chi f_{nn}=n\Bar{f}_{nn},
\end{gather*}
where as usual, the notation $\Bar{f}_{nn}$ indicates that $\cos n\chi\mapsto-\sin n\chi$ and $\sin n\chi\mapsto\cos n\chi$. It is then clear that, dropping the $\epsilon$ factors, 
\begin{gather*}
    \cos n\chi~ \mathrm{component~of~II} \iff -\frac{1}{2}\sin n\chi ~\mathrm{component~of~III} \\
    \sin n\chi~ \mathrm{component~of~II} \iff \frac{1}{2}\cos n\chi ~\mathrm{component~of~III}. 
\end{gather*}
We have thus shown that in fact the equations are no different, and we may safely drop the two components of II. \par
Thus in summary, equation II allows a solution for $B_{\theta n}$ to be found at all orders in terms of $p_n$ and $\Delta_{n-1}$ (and lower order functions), constituting $n-1$ constraint equations. For a diagramatic representation, see Fig. \ref{fig:aniIIeqDiag}.

\begin{figure}
    \centering
    \includegraphics[width=0.55\textwidth]{figures/Chapter3/aniIIeqDiag.jpg}
    \caption{\textbf{Diagram for equation II$^n$.} The green shaded circle represents the function that one should solve the equation for ($\Delta_n$). The arrows indicate the leading order of the functions needed to find a solution (broken lines refer to the special case of $B_{\theta n+1,0}$).}
    \label{fig:aniIIeqDiag}
\end{figure}

\subsubsection{Equation III}
\paragraph{Order $\epsilon^0$}
\begin{align*}
    B_0\frac{\mathrm{d}}{\mathrm{d}\phi}\left[B_{\psi0}(1-\Delta_0)\right]=&B_0B_{\alpha0}B_1p_1+B_0^2B_{\alpha0}p_2-\frac{1}{2}B_{\alpha0}B_2\Delta_0+B_0B_{\alpha1}(1-\Delta_0)-\\
    &-\frac{1}{4}B_\alpha0B_1\Delta_1
\end{align*}
Looking at the three harmonic components, we might obtain expressions for the pressure $p_2$. The 0th harmonic reads,
\begin{align}
    B_0B_{\alpha0}p_{20}^C=&\left[B_{\psi0}(1-\Delta_0)\right]'+B_{\alpha1}(\Delta_0-1)+\frac{1}{2}\frac{B_{\alpha0}}{B_0}B_{20}^C\Delta_0-\frac{1}{2}B_{\alpha0}B_{11}^Cp_{11}^C+\nonumber\\
    &+\frac{B_{\alpha0}}{8B_0}B_{11}^C\Delta_{11}^C,
\end{align}
with the other harmonics given by,
\begin{align}
    p_{22}^C=\frac{1}{8B_0^2}\left(4B_{22}^C\Delta_0-4B_0B_{11}^Cp_{11}^C+B_{11}^C\Delta_{11}^C\right)
\end{align}
and,
\begin{align}
    p_{22}^S=\frac{1}{8B_0^2}\left(4B_{22}^S\Delta_0+B_{11}^C\Delta_{11}^S\right).
\end{align}
So these equations give algebraic closed forms for the pressure harmonic coefficients to order $p_2$ in terms of lower order pressure and anisotropy $\Delta$, as well as $B_{\psi0}$. Note that in the oth harmonic situation one could interpret the equation as an ODE for the $B_{\psi0}$ function, which is at this point otherwise free. However, this involves not only solving an ODE instead of simply performing an algebraic operation, but it will also prove not to be the best way to think about it.

\paragraph{Higher order}: let us now quickly move on to the most general $\epsilon^{n-2}$ case. In order to analyse such an order most efficientlly, we shall, as we did with II, rewrite equation III in a more convenient way. A simple rewriting shows,
\begin{equation}
    \frac{B_\alpha}{B^2}\partial_\psi p_\perp=(\partial_\phi+\Bar{\iota}\partial_\chi)\left[B_\psi(1-\Delta)\right]+(\Delta-1)(\partial_\psi B_\alpha-\Bar{\iota}'B_\theta)+\frac{1}{2}B^2B_\alpha\Delta\partial_\psi\left(\frac{1}{B^2}\right). 
\end{equation}
From this form of the equation it is evident that we may in fact use equation III to arbitrary high order in order to obtain an expression for $p_n$ in terms of $B_{\psi n-2}, \Delta_{n-1}$ and $B_{\theta n-2}$. This therefore constitutes $n+1$ equations at order $\epsilon^{n-2}$, precisely giving an expression for $p_n$ (see Fig. \ref{fig:aniIIIeqDiag} for a diagram). Just for completeness, we shall write,
\begin{equation}
    B_{\alpha0}B_0\frac{n}{2}p_{n,m}=\left[B_{\psi n-2,m}(1-\Delta_0)\right]'+\Bar{\iota}_0(1-\Delta_0)m\Bar{B}_{\psi n-2,m}+\dots \label{eq:IIIAnGen}
\end{equation}

\begin{figure}
    \centering
    \includegraphics[width=0.6\textwidth]{figures/Chapter3/aniIIIeqDiag.jpg}
    \caption{\textbf{Diagram for equation III$^n$.} The green shaded circle represents the function that one should solve the equation for ($p_{n+1}$). The arrows indicate the leading order of the functions needed to find a solution.}
    \label{fig:aniIIIeqDiag}
\end{figure}

\subsubsection{Summary anisotropic construction}
From the anisotropic pressure force balance equation we obtained three sets of constraint, which had to be solved for different functions at different orders. These are summarised in Table \ref{tab:countingQSAnaxis}.

\begin{table}[]
    \centering \hspace*{-.5cm}
    \begin{tabular}{|c||c|c|c|c|}
        \hline
    Eqn. & Order & Solve for\dots & in terms of\dots & Nb. eqns \\ \hline\hline
    I$^n$ & $n$ & $\Delta_n$ & $p_n,\Delta_{n-1}$ & $n+1$ \\\hline
    II$^n$ & $n$ & $B_{\theta n}$ & $p_n,\Delta_{n-1},B_{\theta n-1}$ & $n-1$ \\
    & EVEN & $B_{\theta n0}$ & $p_{n-1},\Delta_{n-1},B_{\theta n-1}$ & (1) \\\hline 
    III$^{n-2}$ & $n-2$ & $p_n$ & $B_{\psi n-2},\Delta_{n-1}, B_{\theta n-2}$ & \\
      &   &   & $p_{n-1}$ & $n+1$ \\ \hline
    \end{tabular}
    \caption{Counting of equations and degrees of freedom. each column shows: the label of equations, the order of expansion, what the equations are solved for, in terms of what other functions they are expressed, and the number of consraints (or independent equations) they amount to. We have included the slightly different nature of the $B_{\theta n0}$ function.}
    \label{tab:countingQSAnaxis}
\end{table}
\par
Briefly stated, we are able to construct solutions for $\Delta$, $p$ and $_{\theta}$, with seemmingly enough degrees of freedom. However, in order to perform an accurate counting we shall propose a construction that wold systematically, to all orders solve the expansion problem. As we shall see in the next subsection, this is not a trivial business even if it might seem so.

\subsection{Complete anisotropic near-axis construction}
In order to come up with a successful order-by-order construction, we should detailedly analyse the functions and equations as they appear in the magnetic and anispotropic force balance equations. As a prelude, let us make a tentative count of the number of free functions and constraint equations, to see if the overdetermination issues that occurred in the magnetostatic case prevail for anisotropic pressure. From the previous sections, we were able to find equations for each of $X,~Y,~Z,~B_\psi,~B_\theta,~p$ and $\Delta$ at every order, leaving only $Y_{n0}$ and $B_{\psi n0}$ functions free. Just to remind the reader, the equations were labelled $J$, $C_\perp$, $C_b$, I, II and III. This rough counting does therefore suggest that, in the anisotropic force balance case, the near-axis construction is not limited to the first few orders, but it can be in principle carried to arbitrarily high order. \par
The reason why we called such a counting a tentative one is because, as things stand, we have not explicitly prescribed a way to orderly and self-consistently construct a solution. For such a construction to be valid, it should allow us to, in some prescribed way, concoct the solution to order $n+1$ given some order $n$. This requires both an understanding of how different functions get involved at different orders, and how they are mutually related. \par
All the information that may be required for this systematic construction is in principle included in Tables \ref{tab:countingQSJCaxis} and \ref{tab:countingQSAnaxis}. However, all of those separate pieces of information ought to be brought together, and we should do so in a way that makes it possible to figure relations and dependencies out. With clarity in mind, we represent these relations with the help of  the diagram shown in Fig. \ref{fig:loopFunAna}. This representation shows the information required to be known in order to find a given function, all according to the equations gathered in Tab. \ref{tab:countingQSJCaxis} and \ref{tab:countingQSAnaxis}. Note the parallel with the magnetostatic case in the scalonated way in which the different orders of the functions have been presented.  \par
\begin{figure}
    \hspace*{+0.5cm}\includegraphics[width=0.9\textwidth]{figures/Chapter3/anisLoop.jpg}
    \caption{\textbf{Function dependency from equations for anisotropic expansion.} The diagram shows the function dependency as governed by the equations obtained in Tabs. \ref{tab:countingQSJCaxis} and \ref{tab:countingQSAnaxis}. The darker circles represent the order of the functions that come to play at the same time according to those equations. The arrows flow from those functions needed to be known to those functions that are to be solved. The darker lines show the main difficulty of this accounting, what we refer to as the \textit{loop}. The broken line indicates that given relation only holds every other order, and only through the $B_{\theta n0}$ component. }
    \label{fig:loopFunAna}
\end{figure}
The diagram in Fig. \ref{fig:loopFunAna} has a main feature of conflict: a \textit{loop} highlighted with thicker black arrows. This close cycle indicates that the three functions depend on each other through the set of equations $C_\perp$, II and III. In fact from those equations we see that: $p_n$ depends on $B_{\psi n-2}$ (see Tab. \ref{tab:countingQSAnaxis}), $B_{\psi n-2}$ depends on $B_{\theta n}$ (see Tab. \ref{tab:countingQSJCaxis}), and finally $B_{\theta n}$ depends on $p_n$ (see Tab. \ref{tab:countingQSAnaxis}). \par
Thus, if we want to be successful in constructing a systematic order-by-order expansion, it is paramount that we undo such a loop. I.e., we need to come with some equations that allows to solve for each of these functions at a time. To do so, the most straightforward approach is to use two of the equations to eliminate two of the functions from the other equation, so as to obtain an equation involving only one of the functions. With such an equation, the solution would then be used to construct the other two functions. Though algebraically involved, such a substitution should otherwise be straightforward. Let us carefully see what happens when doing so at some order $n$. \par
We shall choose $B_{\theta n}$ to be our solve-for candidate. In that case, we need to get rid of $p_n$ and $B_{\psi n-2}$ from equation II. Start with the equation for $B_{\psi n-2}$; from (\ref{eq:CpBpCBtS}) and (\ref{eq:CpBpSBtC})
\begin{gather*}
    B_{\psi n-2,m}^S=\frac{n}{2m}B_{\theta n,m}^C+\dots \\
    B_{\psi n-2,m}^C=-\frac{n}{2m}B_{\theta n,m}^S+\dots
\end{gather*}
where the dots depend generally on $X_{n-1},~Y_{n-1},~Z_{n-1},~B_{\psi n-3}$ and $B_{\theta n-1}$. The harmonic components of $p_{nm}$ can be written using (\ref{eq:IIIAnGen}) as,
\begin{gather*}
    B_{\alpha0}B_0\frac{n}{2}p_{n,m}^C=\left[B_{\psi n-2,m}^C(1-\Delta_0)\right]'+\Bar{\iota}_0(1-\Delta_0)mB_{\psi n-2,m}^S+\dots \\
    B_{\alpha0}B_0\frac{n}{2}p_{n,m}^S=\left[B_{\psi n-2,m}^S(1-\Delta_0)\right]'-\Bar{\iota}_0(1-\Delta_0)mB_{\psi n-2,m}^C+\dots 
\end{gather*}
where the dots represent some combination of $ \Delta_{n-1}$,$~p_{n-1}$, $B_{\theta n-2}$ and lower. Putting these two sets of equations together,
\begin{gather*}
    B_{\alpha0}B_0p_{n,m}^C=-\frac{1}{m}\left[B_{\theta n,m}^S(1-\Delta_0)\right]'+\Bar{\iota}_0(1-\Delta_0)B_{\theta n,m}^C+\dots \\
    B_{\alpha0}B_0\frac{n}{2}p_{n,m}^S=\frac{1}{m}\left[B_{\theta n,m}^C(1-\Delta_0)\right]'+\Bar{\iota}_0(1-\Delta_0)B_{\theta n,m}^S+\dots 
\end{gather*}
which is equivalent to writing,
\begin{equation*}
    B_{\alpha0}B_0p_{n,m}=-\frac{1}{m}\left[\Bar{B}_{\theta n,m}(1-\Delta_0)\right]'+\Bar{\iota}_0(1-\Delta_0)B_{\theta n,m}+\dots 
\end{equation*}
where now the dots represent some combination of $X_{n-1},~Y_{n-1},~Z_{n-1},~\Delta_{n-1},~p_{n-1}$, as well as $B_{\psi n-3}$ and $B_{\theta n-1}$. \par
As a final step, we should substitute $p_{nm}$ in the original equation II. It is evident from such a substitution that all the terms that involve the function $B_{\theta nm}$ exactly cancel! So for every value of $m$ two in principle independent equations remain. These serve as additional constraints on the lower order functions represented by the dots: $X_{n-1},~Y_{n-1},~Z_{n-1},~\Delta_{n-1}$ and $ ~p_{n-1}$, as well as $B_{\psi n-3}$ and $B_{\theta n-1}$. \par
The precise cancellation of the order $n$ $B_\theta$ terms occurs systematically at all orders. As a result, we obtain $n$ additional constraints associated to the $n-1$ functions just mentioned. This is the number of constraints in II. Now, because at every order, from this procedure $B_{\theta n}$ drops, then it is also true that in the previous order so did $B_{\theta n-1}$.\todo{Assumiing that they do not systenmatically drop out as well} Thus, naturally we shall use the $n$ constraint equations (at least in part) to solve for $B_{\theta n-1}$. These equations with the suppressed higher order $B_{\theta n}$ will be referred to as \textit{looped} II equations for obvious reasons. \todo{Could we write this \textit{looped} version of the equations as a non-expanded equaiton? Is there any form of then equations that allows for that?}  \par
The $m=0$ case requires special consideration (see for instance the $1/m$ factors). As an example of such special character, see the $B_{\theta n+1 0}$ role as depicted in the diagram of Fig. \ref{fig:loopFunAna} involving a broken black arrow. For odd orders, we showed in the magnetic construction that one of the harmonics of $Y_n$ is to be solved for in a differential equation that contains $B_{\theta n+1 0}$ and $B_{\psi n-2}$. This could in fact be a problem and make the \textit{loop} equations even more complicated, given that $B_{\psi n-1}$ depends on $Y_n$. However, from Tab. \ref{tab:countingQSAnaxis}, it is the case that solving for $B_{\theta n+1,0}$ does only involve $p_n$ and not $p_{n+1}$. Thus, in a sense, the $B_{\theta n+1,0}$ is to a large extent outside the direct complications of the \textit{loop}. \par 
We have not yet answered definitely the question concerning what to do with the \textit{looped} equations. To answer, let us start by looking at the first instance in which this occurs. The first time that we need to deal with a loop is $n=2$. In that case, the free functions available to the self-consistent problem are $Y_{20},~B_{\psi 0}$ and $\Delta_0$ (or $p_0$, depending on interpretation), in addition to the curvature $\kappa$ and torsion $\tau$ describing the magnetic axis. Then, a possible choice would be to solve the \textit{looped} equations for $Y_{20}$ and $B_{\psi 0}$. Doing so would delay the solution to $B_{\theta 3},~p_3$ and $B_{\psi1}$ into the next order. \par
In that order we would expect to find 3 self-consistent \textit{looped} constraints. Because we are at an odd order, one of the equations involves $B_{\theta 40}$. The other two equations would include all lower order functions. So, the natural way to proceed would be to take these two constraint equations and solve them for the so-far unconstraint $B_{\theta3}$\todo{It is an implicit assumption that these do not somehow cancel exactly in a sort of \textit{loop} simplification}. For doing so, we would have to use III and $C_\perp$ to express everything in terms of $B_\theta$, so that we may solve for it. With such a solution for $B_{\theta 31}^{C/S}$, one may then express $p_3$ and $B_{\psi1}$ in a closed form using the appropriate form of $III^1$ and $C_\perp^2$ respectively. With this at hand, we may solve the non-harmonic component of II$^4$ (which we might call II$_0^4$) explicitly for $B_{\theta 40}$, to finally be able to solve the ODE for one of the components of $Y_3$. \par
This set of steps would be the correct way of approaching this order if the first two constraint equations would not contain the component of $Y_3$ that involves (through the ODE) the $B_{\theta 40}$ and $B_{\psi 11}$ component. If they do have it, then the set of three equations would have to be solved simultaneously for the three functions $B_{\theta 40},~B_{\theta31}^C$ and $B_{\theta31}^S$, to be then able to solve the ODE for the appropriate $Y_3$ component through $C_\perp^3$. In all this, and without looking in more detail at the form of the equations, the existence of solutions is simply hypothesised (as is at this point that no other exact cancellation will occur).\todo{To be given more thought towards the future} \par
The procedure certainly sounds complicated (and even so more when one considers explicitly all the implicit dependencies), and likely numerically intense. However, there seems to be (without checking the solubility of the equations in more detail) a generalised way of dealing with the loops. We briefly summarise it:
\begin{itemize}
    \item if the order $n$ is odd, then the II$^{n+1}$ equations should be used (in conjuction with III and $C_\perp$) to solve for $B_{\theta n}$ and $B_{\theta n+1 ,0}$. 
    \item if the order $n$ is even, then the two of the II$^{n+1}$ equations shall be used to self consistently solve for $Y_{n0}$ and $B_{\psi n-2 ,0}$ (similarly to how it was done for $n=2$), and the other remaining $n-2$ equations should go into solving $B_{\theta n}$ (excluding $B_{\theta n,0}$ which had been solved in the previous order).
\end{itemize} 
Having `resolved' the complications associated to the \textit{loop}, we may now propose, following the indications above, a final construction for an order-by-order solution for the near-axis quasisymmetric field expansion. We shall now use the same form of proceeding as was introduced for the magnetostatic case. \par
First, we should know to a given order how do the different functions come into play. The question that needs to be addressed is: how can we add higher orders of the expansion in such a way that the problem formulated is self consistent? The answer is shown in Fig. \ref{fig:ConstructNAAnis}, and we have included a color code, as well as a number of arrows to show dependencies. \par
\begin{figure}
    \hspace*{+0.5cm}\includegraphics[width=0.9\textwidth]{figures/Chapter3/AnisfunOrder.jpg}
    \caption{\textbf{Consistent order of functions.} Order of functions that ought to be simultaneously solved for. The color code represents the order in which the functions are solved for: red - first to be solved using the \textit{looped} form of II, dark orange, bright orange, yellow and pale yellow. The blue color represents the introduction of free functions at even orders that are to be solved self consistently. The dashed arrow and reddish colored part of $B_{\theta n+1}$ represent that for odd orders, the 0 harmonic term of the next order is to be solved simultaneously as well. The arrows show the mutual dependencies, originating from $B_{\theta n}$.}
    \label{fig:ConstructNAAnis}
\end{figure}
Secondly, we should indicate which equations are to be solved to determine which functions and to what order. This collection is shown in Table \ref{tab:eqConstructNAAnis}. \par
\begin{table}[]
    \centering \hspace*{-1cm}
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
    \hline
    MS & $X_n$ & $Y_n$ & $Z_n$ & $B_{\theta n}$ & $B_{\psi n}$ & $p_n$ & $ \Delta_n $ \\ \hline\hline
    0 &  \cellcolor{black} & \cellcolor{black} & \cellcolor{black} & $C^{-1}$ & \small $\Tilde{\mathrm{II}}^3_\mathrm{SC}$ & \cellcolor{GreenYellow}$p_0$ & $\mathrm{I}^0$   \\\cline{2-8}
    1 & $J^1$ & \small $C_b^0$|$\tilde{C}_\perp^1(1)$ & $C_\perp^0$ & $C_\perp^0$ & \small $C_\perp^2$ & \small II$^1$ & $\mathrm{I}^1$ \\\cline{2-8}
    2 &  $J^2$ & \small $C_b^1(2)$|$\Tilde{\mathrm{II}}_\mathrm{SC}^3$ & $C_\perp^1$ &  \small $\tilde{\mathrm{II}}^2(1)|C_\perp^1$ &  \small $C_\perp^3(2)$|$\Tilde{\mathrm{II}}_\mathrm{SC}^5$  & \small $\mathrm{III}^0$ & $\mathrm{I}^2$  \\\hline \hline
    $n=2k$ &  $J^n$ & \small $C_b^{n-1}(n)$|$\Tilde{\mathrm{II}}_\mathrm{SC}^{n+1}$ & $C_\perp^{n-1}$ &  \tiny $\tilde{\mathrm{II}}^n_0(1)|\tilde{\mathrm{II}}^{n+1}|C_\perp^{n-1}(2)$ &  \small $C_\perp^{n+1}(n)$|$\Tilde{\mathrm{II}}_\mathrm{SC}^{n+3}$  & \small $\mathrm{III}^{n-2}$ & $\mathrm{I}^n$  \\\cline{2-8}
    $n+1$ &  $J^{n+1}$ & \small $C_b^{n}$|$\Tilde{C}_\perp^{n+1}(1)$ & $C_\perp^{n}$ &  \small $\tilde{\mathrm{II}}^{n+2}|C_\perp^{n}(2)$ &  \small $C_\perp^{n+2}$ & \small $\mathrm{III}^{n-1}$ & $\mathrm{I}^{n+1}$  \\\hline
    \end{tabular}
    \caption{\textbf{Anisotropic near-axis construction,} Each cell represents the equations that need to be solved to find a function (column) at a given order (row). The equation labels are as follows: $J$ for the Jacobian equation, $C_\perp$ and $C_b$ for the co(ntra)variant perpendicular and $b_0$ components, and I, II and III for the force balance equations. According to the discussion on the \textit{loop}, the notation$\Tilde{\mathrm{II}}$ refers to the \textit{looped} version of the equation, with the underscript SC referring to the self-consistent equation to be solved for $Y_{n0}$ and $B_{\psi n-2,0}$. The numbers in parenthesis denote the number of constraint equations (where no number is given is because they account for the precise number of unknowns in that cell). The green color shows the only free function left in the construction apart from the curvature and torsion of the axis.}
    \label{tab:eqConstructNAAnis}
\end{table}
A couple of words shall be spared to explain the construction depicted in the table and diagrams presented. With both of these tools at hand, we may sketch what the construction would be like. Let us start off with an odd order. Following Fig. \ref{fig:ConstructNAAnis}, one should start off by solving for $B_{\theta n}$, but also $B_{\theta n+1,0}$. The latter, as we saw before, needs to be included in the calculation as it appears in the ODE $\tilde{C}_\perp^n$ that is to be solved for $Y_n$. To solve for these $B_\theta$ harmonics we shall follow Tab. \ref{tab:eqConstructNAAnis}. First, to drop the saturated harmonics following $C_\perp^{n-1}$, to be left with $\Tilde{\mathrm{II}}^{n+1}$. This equation represents the \textit{looped} version of equation II, in which all the functions to order $n$ (and $B_{\psi n-2}$) have been substituted for $B_{\theta n}$ and $B_{\theta n+1,0}$. Note that we may have $B_{\psi n-1 0}$ present in the equations, at this point a free function. The equations needed to peform such a substitution are the ones sharing the row in the table, and two before for $B_\psi$ (note that in a sense we need to \textit{loop} II twice, once to get rid of the higher $B_{theta}$s, and a second time to reespress everything in terms of $B_{\theta n}$). Once $B_{\theta}$ has been solved for, we may follow the indicated flow in the diagram in Fig \ref{fig:ConstructNAAnis}. Constuct $B_{\psi n-2}$ using $C_\perp^{n-1}$ from the table, and continue substituting what we know to construct $Z_n$ and $p_n$, following $\Delta_n$ and $X_n$. With this knowledge an $B_{\theta n+1,0}$, finally $Y_n$ may be solved for. \par
In the case of an even order, the construction needs to change slightly. This is mainly because in addition to solving for $B_{\theta n}$ using the \textit{looped} version of II, we also have to solve self consistently for the functions $Y_{n0}$ and $B_{\psi n-2,0}$. As may be seen from Tab. \ref{tab:eqConstructNAAnis}, this self-consistent equation comes also from the looped version of II. Thus, we could say that the equations would have to be solved simultaneously for functions $B_{\theta n}$ (note that $B_{\theta n 0}$ would have been solved in the previous order), $Y_{n0}$ and $B_{\psi n-2,0}$. Following this, we would follow the arrows in the diagram in an almost identical way to how we did in the odd case to construct the rest of the functions. Noticeably, in this caswe, no ODE would have to be solved to find $Y$ (other than the self-consistent problem that was addressed at the start of this order).  \par
With this construction in our hands, and backed by the Table and diagram, we are now in a position to count in an effective way. From the way we have constructed the solution, it is evident that the problem is not overconstraint, nor is it underconstraint. In fact, there are precisely the same number of constraint equations that need to be solved at each order as the number of functions that appear anew. This is evident from the fact that Tab. \ref{tab:eqConstructNAAnis} is exactly tiled by the available equations, with no gap left in it. One could in addition check that the equation number in the table add up to the appropriate numnber. We add a short equation number reference table (Tab. \ref{tab:countingEqNum}) for ease. \par
\begin{table}[]
    \centering \hspace*{-.5cm}
    \begin{tabular}{|c|c||c|c|}
        \hline
        Eqn. & Nb. eqns&Eqn. & Nb. eqns \\ \hline\hline
    I$^n$ & $n+1$ & $J^n$ & $n+1$\\
    II$^n$ & $n-1$ & $C_b^n$ & $n+1$\\
    III$^{n-2}$ & $n+1$ & $C_\perp^n$ & $2(n+2)$\\\hline
    \end{tabular}
    \caption{\textbf{Number of constraint equations.} Number of total independent constraints associated to each one of the relevant equations.}
    \label{tab:countingEqNum}
\end{table}
So, as far as the counting goes, by relaxing the magnetostatic equilibrium, the near axis expansion avoids, as expected, the overdetermined nature of the near axis expansion from \cite{garrenboozer1991b}. Thus, by explicitly constructing the anisotropic quasisymmetric field around a magnetic axis, we have shown that is a priori possible to continue the expansion to orders higher than two, which has been the classsical limitation. We have to say \textit{a priori} because we have not shown explicitly that the equations that need to be solved at higher order do have a solution, and even that some may not become dependent on each other. This problem is equally present for \cite{garrenboozer1991b}. \par
Despite not being able to use this construction as a definitive proof of the existence of a global solution to quasisymmetry, it however suggests that there is likely a way to construct such globally QS fields. This is diametrically opposite to the current understanding, which incited by \cite{garrenboozer1991b}, is that globally QS solutions do likely not exist (except in truly symmetric cases such as axisymmetry). The view here is in fact an interesting one, as it seems to open up the door to QS, for which a consistent form of force balance is required. In this particular case, a consistent form of anisotropy.\todo{Could we show an example of it working? Perhaps the circular axis is the best candidate as a starting point} \par
\textbf{This naturally takes us to a discussion of the physicality of the construction we have just sketched above. Is it physically meaningful to have a system with a particular form of anisotropy (is there any particular constraint such as a Braginskii-like consideration)? How large does this anisotropy have to be for things to work (could we make it arbitrarily small)? Could we `construct' it in real life using some sort of neutral beam injection? Could other possible forms of force balance also work? }

\section{Circular axis quasisymmetric field}


% Let us now move on to the force balance of interest, in this case $\n{j}\times\n{B}=\nabla\cdot\Pi$.
% \begin{enumerate}
%     \item Equation I:
%     \begin{equation*}
%         \frac{1}{B^2}(\partial_\phi+\Bar{\iota}\partial_\chi)\left(\frac{\Delta p}{B^2}\right)+\frac{1}{B^4}(\partial_\phi+\Bar{\iota}\partial_\chi)p_\perp=\frac{\Bar{\iota}}{2}\frac{\Delta p}{B^2}\partial_\chi\left(\frac{1}{B^2}\right)
%     \end{equation*}
%     which merely relates $p_\perp$ to $\Delta p/B^2$ through $1/B^2$. So, proceeding in an orderly manner,
%     \begin{itemize}
%         \item Order $\epsilon^0$:
%         \begin{equation*}
%             \boxed{B_0 p_{0}+\Delta_0=\mathrm{const}}
%         \end{equation*}
%         where $p$ and $\Delta$ are short hand for $p_\perp$ and $\Delta p/B^2$ respectively. This is $\Tilde{I}^0$ as it appears in (0,7).
%         \item Order $\epsilon^1$:
%         \begin{empheq}[box=\widefbox]{gather*}
%             B_0p_{11}^C+\Delta_{11}^C=\frac{B_{11}^C}{2B_0}\sum_{n=0}^\infty\frac{\Bar{\iota}_0^2-2n^2}{\Bar{\iota}_0^2-n^2}\left(\Bar{\Delta}_{0n}^S\sin n\phi+\Bar{\Delta}_{0n}^C\cos n\phi\right)\\
%             B_0p_{11}^S+\Delta_{11}^S=\Bar{\iota}_0\frac{B_{11}^C}{2B_0}\sum_{n=0}^\infty\frac{n}{\Bar{\iota}_0^2-n^2}\left(\Bar{\Delta}_{0n}^S\cos n\phi-\Bar{\Delta}_{0n}^C\sin n\phi\right)
%         \end{empheq}
%         where we have Fourier series expressed $\Delta_0=\sum_{n=0}^\infty(\Bar{\Delta}_{0n}^C\cos n\phi+\Bar{\Delta}_{0n}^S\sin n\phi)$ to easily manage the derivatives, and exploit the physically required periodicity of the functions. The important point here is that we have a closed form expression relating $\Delta$ and $p$, which in this case involved solving an ODE in $\phi$. This corresponds to $\Tilde{I}^1$ as it appears in  (7,1).
%         \item Higher order: so at order $\epsilon^n$, we expect to have $n+1$ equations that ought to be solved for $\Delta_n$ as function of $p_n$. There is a clear pathway here as to how we should proceed. The sine and cosine terms of the same order are related by similar SHO relation that we observed in $\epsilon^1$, and thus are to be solved the same way (exploiting the convenient $\phi$ Fourier series, and only looking for the particular solution). The constant term (i.e., the zero harmonic) is even easier, as one just needs to integrate w.r.t. $\phi$. Thus the counting goes like $n+1$ equations for $\Delta_n$ and $p_n$. \par
%         As an example of the approach, the $\epsilon^2$ term ($\Tilde{\mathrm{I}}^2$),
%         \begin{align*}
%             (B_0p_{20}^C+\Delta_{20}^C)'&=-\frac{\Bar{\iota}_0}{4}\frac{B_{11}^C}{B_0}(\cancel{4B_0p_{11}^S}+3\Delta_{11}^S)+\frac{(B_{11}^C)^2\Delta_0'}{2B_0^2}+\frac{B_{20}^C}{B_0}\Delta_0'-\\ 
%             &-\frac{B_{11}^C}{2B_0}(2B_0p_{11}^C+\Delta_{11}^C)'
%         \end{align*}
%         and
%         \begin{gather*}
%             \mathcal{A}+2\Bar{\iota}_0(BB_0p_{22}^S+\Delta_{22}^S)+(B_0p_{22}^C+\Delta_{22}^C)'=0\\
%             \mathcal{B}-2\Bar{\iota}_0(BB_0p_{22}^C+\Delta_{22}^C)+(B_0p_{22}^S+\Delta_{22}^S)'=0
%         \end{gather*}
%         and $\mathcal{A}$ and $\mathcal{B}$ are a combination of lower order functions of $p$ and $\Delta$,
%         \begin{gather*}
%             \mathcal{A}=\Bar{\iota}_0\left[-\frac{B_{22}^S}{B_0}\Delta_0+\frac{B_{11}^C}{4B_0}(\cancel{4B_0p_{11}^S}+\Delta_{11}^S)\right]-\frac{(B_{11}^C)^2}{2B_0^2}\Delta_0'-\frac{B_{22}^C}{B_0}\Delta_0'+\frac{B_{11}^C}{2B_0}(2B_0p_{11}^C+\Delta_{11}^C)'\\
%             \mathcal{B}=\Bar{\iota}_0\left[\frac{B_{22}^C}{B_0}\Delta_0-\frac{B_{11}^C}{4B_0}(4B_0p_{11}^C+\Delta_{11}^C)\right]-\frac{B_{22}^S}{B_0}\Delta_0'+\frac{B_{11}^C}{2B_0}(\cancel{2B_0p_{11}^S}+\Delta_{11}^S)'
%         \end{gather*}
%     \end{itemize}
%     \item Equation II:
%     \begin{align*}
%         A_\alpha\left(1-\frac{\Delta p}{B^2}\right)+\frac{B_\theta}{B^2}\partial_\phi p_\perp=\frac{B_\alpha-\Bar{\iota}B_\theta}{B^2}\partial_\chi p_\perp       +\frac{B_\alpha-\Bar{\iota}B_\theta}{2}B^2\frac{\Delta p}{B^2}\partial_\chi\left(\frac{1}{B^2}\right)
%     \end{align*}
%     where $A_\alpha=(\partial_\phi+\Bar{\iota}\partial_\chi)B_\theta-\partial_\chi B_\alpha$. 
%     \begin{itemize}
%         \item Order $\epsilon^0$: tautological
%         \item Order $\epsilon^1$: 
%         \begin{empheq}[box=\widefbox]{gather*}
%             B_0p_{11}^S=\Bar{\zeta}(1-\Delta_0)=0 \\
%             B_0p_{11}^C=\Bar{\eta}(1-\Delta_0)+\frac{1}{2}\frac{B_{11}^C}{B_0}
%         \end{empheq}
%         \item Order $\epsilon^2$:
%         \begin{equation*}
%             \boxed{\frac{\mathrm{d}}{\mathrm{d}\phi}\left[B_{\theta20}^C(1-\Delta_0)\right]=\mathcal{J}(p_{11}^S,p_{11}^C,\Delta_{11}^S,\Delta_{11}^C)}
%         \end{equation*}
%         where $\mathcal{J}$ is some convoluted function of lower order $p$ and $\Delta$,
%         \begin{align*}
%             \mathcal{J}=B_{\alpha0}B_{11}^Cp_{11}^S-\frac{B_{\alpha11}^S}{4B_0}\left[B_{11}^C(\Delta_0-2)+2B_0(B_0p_{11}^C+\Delta_{11}^C)\right]+\\
%             +\frac{B_{\alpha0}}{4B_0}B_{11}^C\Delta_{11}^S+\frac{1}{2}B_{\alpha11}^C(B_0p_{11}^S+\Delta_{11}^S)
%         \end{align*}
%         The equation might be thought of as an equation to be solved for $B_{\theta20}^C$ ($\Tilde{\mathrm{II}}^2$). Looking at the solubility condition of such an ODE (i.e. requiring the RHS of the equation to have a vanishing $\phi$ integral), one may show that $B_{\alpha11}^S=0$, and thus $\Bar{\zeta}=0$ (as chosen for the $B$ field harmonic). In fact,
%         \begin{equation*}
%             \boxed{B_{\theta20}^C(1-\Delta_0)=\Bar{B}_{\theta20}-\Bar{\iota}_0B_{\alpha0}\frac{\Bar{\eta}B_{11}^C}{4B_0}\sum_{n=0}^\infty\frac{1}{\Bar{\iota}_0^2-n^2}\left(\Bar{\Delta}_{0n}^S\sin n\phi+\Bar{\Delta}_{0n}^C\cos n\phi\right)}.
%         \end{equation*}
%         where $\Bar{B}_{\theta20}$ is a constant (from the integration).
%         \par
%         As a matter of fact, there are two additional equations (corresponding to the harmonics $\cos2\chi$ and $\sin2\chi$), involving $B_{\theta22}$. From the Jacobian we know that these must be zero, and then, the remaining equations turn out to be equivalent to constraints for $p_2$ from Equation III as we will see. 
%         \item Higher order: thus to order $\epsilon^n$, the equations obtained may be thought of to determine the $\boxed{B_{\theta n}}$ components. In fact, we shall note that we will have $n-1$ independent equations, for the same number of undetermined components of $B_{\theta n}$. The equations involve $\{p_n,\Delta_{n-1},B_n\}$, and we will have to generally solve for terms of the form of the LHS of the $\epsilon^2$ equation shown.
%     \end{itemize}
%     \item Equation III:
%     \begin{align*}
%         A_\psi\left(1-\frac{\Delta p}{B^2}\right)+B_\psi(\partial_\phi+\Bar{\iota}\partial_\chi)\left(\frac{\Delta p}{B^2}\right)-\frac{1}{2}B^2B_\alpha\frac{\Delta p}{B^2}\partial_\psi\left(\frac{1}{B^2}\right)+J\partial_\psi p_\perp=0
%     \end{align*}
%     where $A_\psi=-\Bar{\iota}\partial_\chi B_\psi-B_\theta\Bar{\iota}'+(\partial_\psi B_\alpha-\partial_\phi B_\psi)$. 
%     \begin{itemize}
%         \item Order $\epsilon^0$:
%         \begin{empheq}[box=\widefbox]{align*}
%             \left[B_{\psi0}(1-\Delta_0)\right]'=B_{\alpha20}^C(\Delta_0-1)+\frac{1}{2}\frac{B_{\alpha0}}{B_0}B_{20}^C\Delta_0-B_{\alpha0}B_{11}^Cp_{11}^C-2B_0B_{\alpha0}p_{20}^C-\\
%             -\cancel{\frac{1}{2}B_0B_{\alpha11}^Sp_{11}^S}-\frac{B_{\alpha11}^C}{4B_0}\left[B_{11}^C(2-3\Delta_0)+2B_0(B_0p_{11}^C-\Delta_{11}^C)\right]+\\
%             +\frac{B_{\alpha0}}{4B_0}B_{11}^C\Delta_{11}^C+\cancel{\frac{1}{2}B_{\alpha11}^S\Delta_{11}^S}
%         \end{empheq}
%         Now, we shall interpret this equation as an equation defining $p_{20}^C$, as a function of lower order $p_\perp$ and $\Delta$, and the free function $B_{\psi0}$. This latter freedom does also exist in the context of the magnetostatic equilibrium (note that we could opt for $p_{20}^C$ as a free function instead, but then one would need to integrate the equation to obtain the the other function). In a similar way, one may solve the other two equations for $p_{22}^C$ and $p_{22}^S$,
%         \begin{empheq}[box=\widefbox]{align*}
%             p_{22}^C=\frac{1}{8B_0^2B_{\alpha0}}\left\{8B_0B_{\alpha22}^C(\Delta_0-1)+4B_{\alpha0}B_{22}^C\Delta_0-4B_0B_{\alpha0}B_{11}^Cp_{11}^C+\right.\\
%             +\cancel{2B_0^2B_{\alpha11}^Sp_{11}^S}+B_{\alpha0}B_{11}^C\Delta_{11}^C-B_{\alpha11}^C\left[B_{11}^C(2-3\Delta_0)+2B_0(B_0p_{11}^C-\right.\\
%             \left.\left.-\Delta_{11}^C)\right]-\cancel{2B_0B_{\alpha11}^S\Delta_{11}^S}\right\}
%         \end{empheq}
%         \begin{empheq}[box=\widefbox]{align*}
%             p_{22}^S=\frac{1}{8B_0^2B_{\alpha0}}\left\{8B_0B_{\alpha22}^S(\Delta_0-1)+4B_{\alpha0}B_{22}^S\Delta_0-\cancel{4B_0B_{\alpha0}B_{11}^Cp_{11}^S}-\right.\\
%             -\cancel{2B_0^2B_{\alpha11}^Cp_{11}^S}+B_{\alpha0}B_{11}^C\Delta_{11}^S-B_{\alpha11}^S\left[\cancel{B_{11}^C(2-3\Delta_0)+2B_0(B_0p_{11}^C-}\right.\\
%             \left.\left.\cancel{-\Delta_{11}^C)}\right]\cancel{+2B_0B_{\alpha11}^C\Delta_{11}^S}\right\}
%         \end{empheq}
%         \item Higher order: one may similarly proceed to higher, to obtain closed form expressions for all the Fourier components of $\boxed{p_{n+2}}$. Note that these forms/expressions will express $p_{n+2}$ in terms of $\{B_{\psi n},p_{n-1},\Delta_{n-1},B_{n+2}\}$. No differential equation needs to be solved for $p_{n+1}$ but simply read the solution out form each equation.
%     \end{itemize}
% \end{enumerate}

